Editing Motion Graphics Video via Motion Vectorization and Transformation

Motion graphics videos are widely used in Web design, digital advertising, animated logos and film title sequences, to capture a viewer's attention. But editing such video is challenging because the video provides a low-level sequence of pixels and frames rather than higher-level structure such as the objects in the video with their corresponding motions and occlusions. We present a motion vectorization pipeline for converting motion graphics video into an SVG motion program that provides such structure. The resulting SVG program can be rendered using any SVG renderer(e.g. most Web browsers) and edited using any SVG editor. We also introduce a program transformation API that facilitates editing of a SVG motion program to create variations that adjust the timing, motions and/or appearances of objects. We show how the API can be used to create a variety of effects including retiming object motion to match a music beat, adding motion textures to objects, and collision preserving appearance changes.

==> Makefile <==
# make -f Makefile_pdflatex

R = main

pdf: $(R).pdf

$(R).bbl: $(R).bib
	pdflatex $(R)
	bibtex $(R)
	pdflatex $(R)

$(R).pdf: *.tex $(R).bbl
	pdflatex $(R)



notes:
	pdflatex "\def\MakeWithNotes{}\input{$(R)}"

wo:
	pdflatex "\def\MakeWithoutNotes{}\input{$(R)}"

clean:
	rm -f $(R).log $(R).aux $(R).bbl $(R).blg $(R).out



==> applications.tex <==
\maneesh{------Old Text below this point-------}
\section{Embedded Domain-Specific Language} % Rename to program transformations? Demonstrated examples?
\label{sec:apps}
% Describe in terms of applications rather than what the problem that needs to be solved

% What should be emphasized?
% - Every application must be reproducable/implementable, also within context of the program

% SVG in, SVG out (operations that are applied to parts of the input SVG and produces new SVGs as output)
% "Program transformation"
% some can be short, others need to be in more detail

% In CVPR, this section is similar to their Evaluation section
% we have this program representation -> it allows these things

% Need some context on why this is important for readers to know about
%  - RoughCut paper

In this section, we introduce an embedded domain-specific language (DSL) that encapsulates primitive operators which users can apply to programs at the object-level. We first describe the different datatypes in our DSL. We then describe several semi-automated program transformations built with these operators that accomplish various motion graphics editing tasks. 
% \sharon{This sentence feels convoluted, any suggestions on improvements?}

\sharon{I'm not sure if the part below is exactly a decription of ``datatypes,'' but I thought it may be important to decribe as we refer to each of these program parts in our methods and transformations.}
Our system outputs SVG + SMIL programs. A program contains any number of objects as well as metadata about the overall composition. The composition metadata includes
\begin{itemize}
    \item the total number of frames in the video;
    \item the backgrond appearance at each frame;
    \item and the dimensions of the video.
\end{itemize}

\sharon{Thoughts on describing the objects this way?}
We represent objects as a collection of fields, specifically including
\begin{enumerate}
    \item the object appearance;
    \item the local motion parameters (scale, rotation, skew, position);
    \item the global motion parameters (scale, rotation, skew, position);
    \item and the $z$-index.
\end{enumerate}

\subsection{Object-level methods}
\jiaju{Do we want to say something like Program Transformation or Object-level API?}

% \sharon{Are there specific formats for describing the program + operators? I've seen some systems papers which just list out methods in their API as bullet points (maybe the method name is formatted in a monospace font) so that is what I have so far.}

We introduce a lightweight API of object-level methods. There are two types of methods: \textbf{state queries} and \textbf{operators}. A query retrieves information about the object at a particular frame. An operator takes in an entire object and a time range specified by a start frame and end frame, along with any other additional necessary parameters. The operator then makes the desired modifications to the object within that time range in place. Methods of both types are described below.

\subsubsection{State queries}
\begin{description}
    \item[\texttt{query(obj, eventType, frame)}:] Given an input object \texttt{obj}, this function retrieves its relevant information based on \texttt{eventType} at \texttt{frame}. Possible events are: \texttt{collision}, \texttt{causality}, etc. \jiaju{I wrote this based on my understanding of what we discussed. Feel free to update!}
\end{description}

\subsubsection{Operators}
\begin{description}
    \item[\texttt{freezeFrame(obj, freezeStartFrame, freezeLength)}:]
    \jiaju{I looked into After Effect and Premiere and it should be called freeze frame instead of hold frame} \
    Freeze the frame \texttt{freezeStartFrame} for the duration of \texttt{freezeLength}, which is in the units of frames.

    \item[\texttt{retime(obj, startFrame, endFrame, easingFn)}:]Apply easing function \texttt{easingFn} to \texttt{obj}'s time from \texttt{startFrame} to \texttt{endFrame}. \jiaju{Should we discuss edge cases here (e.g. endFrame is longer than the duration of the animation), also for other operators as well?}
    
    \item[\texttt{adjustLocalMotion(obj, startFrame, endFrame, fn)}:]
    Apply function \texttt{fn} to \texttt{obj}'s local motion from \texttt{startFrame} to \texttt{endFrame}.

    \item[\texttt{adjustGlobalMotion(obj, startFrame, endFrame, fn)}:]
    Apply function \texttt{fn} to \texttt{obj}'s global motion from \texttt{startFrame} to \texttt{endFrame}.

    \item[\texttt{changeAppearance(obj, newAppearance, startFrame, endFrame)}:]
    Changes the appearance of object \texttt{obj} to \texttt{newAppearance} for the time range \texttt{start\_frame} to \texttt{end\_frame}.
    \jiaju{Is changeAppearance a low-level operator or an application, if adjustLocalMotion is needed for the object to hit the right collision points?}
\end{description}

% \sharon{Everything above this comment is new + separate from things below this comment. I'm thinking of using the above content as an outline for the final text, and anything below may be encapsulated into another subsection called ``Program transformations" or something of that sort.}


\subsection{Program Transformations}
We now describe several program transformations that perform motion graphics editing tasks. These program transformations are built with the state queries and operators introduced above, and all 
take as input a SVG + SMIL program, apply transformations, and output a new SVG + SMIL program.


\subsubsection{Animation retiming}
Retiming is a common task in video editing~\cite{}. The user can perform a variety of retiming tasks by passing various easing functions and other parameters into the \texttt{retime()} operator.
\begin{description}
    \item[Video time remapping]
    To remap the time of an individual object, pass into \texttt{retime()} an easing function $f(t)=a \cdot t$, where $a$ is the linear remapping factor (e.g. $a=2$ speeds up the animation by 2, and $a=\frac{1}{3}$ slows down the the animation by 3). The easing function is applied to the time region in between \texttt{startFrame} and \texttt{endFrame}. To remap the video as a whole, run \texttt{retime()} on every object with the same easing function, and set \texttt{startFrame} and \texttt{endFrame} to the first and last frame of the entire video respectively.

    \item[Retiming to music beats]
    With a piece of music provided, first extract beats in the units of frames. For an individual object, repeatedly apply \texttt{retime()} with \texttt{startFrame} and \texttt{endFrame} set to two consecutive beat frames. Any easing function, such cubic ease in and quintic ease out, can be used. Repeat this process for all objects to retime the entire video to the beats. The video or an object's animation can be remapped first to hit full beats.
    
    \item[Animating on 1s, 2s, 3s, and $n$s] 
    Animating on 1s, 2s, 3s, or $n$s is an animation technique that holds a frame once, twice, three times, or $n$ times. To achieve this effect, a step function can be used as the easing function for \texttt{retime()}. Alternatively, this can be achieved by applying the \texttt{freezeFrame()} operator on every $n$th frame.
    % The user can also apply various motion filters to the animated elements. Animating on 1s, 2s, and 3s is an animation technique that holds a frame once, twice, or three times (CITE). By applying our filter, the user can convert between arbitrary number of frame holds, such as converting a motion animated on 3s to a new motion animated on 6s.
    \jiaju{I realized animating on ns can be achieved by passing in a step function, as demonstrated in \href{https://developer.mozilla.org/en-US/docs/Web/CSS/animation-timing-function}{\underline{this link}}.}
\end{description}


\subsubsection{Motion filters} Besides edits in the time domain, changes can also be made in the spatial domain via the \texttt{adjustLocalMotion()} and \texttt{adjustGlobalMotion()} operators.
\begin{description}
    \item[Cartoon animation filter]
    We adopted the cartoon animation filter proposed by Want et al.~\cite{}. This filter can be passed in as a function to \texttt{adjustGlobalMotion()} for an object to create the animation effects of anticipation and follow through~\cite{}. \jiaju{Is adjustGlobalMotion only changing the translation? Do we want an operator that changes the other transformations too?}
    \item[Motion textures]
    This can be achieved by passing in various functions to \texttt{adjustLocalMotion()}. \jiaju{A short placeholder for now. Will expand as we look into this.}
\end{description}


\subsubsection{Visual element substitutions} 
% Preserving collisions
% Part of replacing objects?
We perform \textit{object substitutions} by swapping out visual appearances of various objects. This can be done simply by pointing each object appearance attribute to a new file, but the resulting video may not preserve certain inter-object interactions. A common object interaction in motion graphics is when two objects have a point of physical contact (\eg collisions, resting atop one another). The aforementioned vanilla substitution will likely not preserve such events if the new object has a significantly different contour than the original object. We now describe a procedure to preserve contacts and collisions between two objects when either is replaced.

\subsubsection{Detecting contact points.} A meaningful contact points $(x, y, t)$ is defined as a point of overlap $(x, y)$ at time $t$ between two entities. In the case that two objects are involved in the contact, we require that (1) the total overlap between the two objects at time $t$ is minimal and (2) at least one of the objects experiences a sign change in velocity in the $x$ or $y$ direction. In the case that a single object is involved in the contact (\eg the object bounces off an ``invisible" boundary), we only use requirement (2).

To detect all collision points in frame $F_t$, we take the boundaries of all objects in that frame, dilate them and look for intersections. The boundary information is obtained from rendering out each object according to its appearance and parameters in our video program. This information also allows us to exclude overlaps as contact points. We look at the average velocity in the $x$ and $y$-directions for a span of $n$ frames before and after $t$. If the sign of the average velocity is different before and after $t$ (we use three ``signs" here: $+$, $-$ and $0$), then we register a directional change.
\sharon{Add this to code.} The contact points for each shape are then written into the program.

\subsubsection{Local adjustments to preserve object contact.}

\subsubsection{Automatic aspect ratio adjustment}
\begin{enumerate}
    \item Grouping. Group visual elements and their animations together. 
    % \jiaju{should we talk about causality detection here?}
    \item Anchoring. Anchoring a visual element is a common technique employed in responsive web and UI design and can be found in industry standard tools like Figma and Sketch.
    The user can specify different anchors for translation and scaling.
    \item \jiaju{Preserving collisions is also needed here?}
    \item Moving window. The user can specify a target object to follow, and the moving window moves with it.
\end{enumerate}

\subsubsection{Program substitutions} % Find a different name here
\begin{enumerate}
    \item \jiaju{not sure exactly what goes in here for now}
    \item Removing visual elements
    \item Mix and match different animations
\end{enumerate}

\subsubsection{Format conversions}
\begin{enumerate}
    \item \jiaju{I don't think this section should be in here, and I also wonder where we should put it/do we need it?}
    \item After Effects: a \program $s$ can be imported into After Effects via an ExtendScript script. The imported \program can then be further edited within After Effects and output to various formats.
    \item Blender: a \program $s$ can be imported into Blender by using its python API. Similarly, the imported motion file can be further edited into various formats.
\end{enumerate}


==> diff_comp.tex <==
\subsection{Differentiable Compositing}\label{sec:diffcomp}

The process of executing our programs involves rendering shapes out a frame, and compositing them in the order of their specified $z$-indexes. We use the standard compositing equation
\begin{equation}
  I = \alpha \cdot I_\text{FG} + (1 - \alpha) \cdot I_\text{BG},
\end{equation}
where $I$ is the resulting composite image, $I_\text{FG}$ is the current layer and $I_\text{BG}$ is the background image. \sharon{Look up the standard terminology for each of these variables.} One issue is that this process is not differentiable, as the layering of objects is discrete.

Reddy~\etal~\cite{} introduce a differentiable compositing process along with a compatible optimization framework. To address the discrete layering issue, the method colors each pixel value with a weighted average of the RGB value at the corresponding pixel position in all the composite layers. The weight of each layer is a softmax over all the layer alpha values at that position. With this modification, they introduce a procedure that can optimize the placements of various templates to match a target pattern. To ameliorate the issue of small spatial gradients, they use a pyramid visual loss. We refer the reader to their paper for more details.

In order to compute the motion information for our programs, we require the orientations and layering order of each object. Given a target frame and a set of objects which appear in that frame, we can adapt the differentiable compositing method to include the $x$-scale, $y$-scale, rotation, $x$-skew, $y$-skew and centroid position of each object at a fine-grained level.

Although the image pyramid in the differentiable compositing loss helps increase the region of influence of spatial gradients, we have found that it still fails to converge to a global minimum when objects are very far from their target positions. Moreover, the optimization may also converge to a local minimum on the other parameters. In order to improve the converged solution, we compute initialize the optimization variables 

==> diff_comp_v2.tex <==
\subsection{Differentiable compositing}
Differentiable compositing (DC) is an optimization technique that was
originally designed to decompose a graphic pattern comprised of
discrete elements that may partially occlude one another, into 
layered representation~\cite{}. 
As input it takes a {\em target} pattern image $T$, and a set of {\em source} element
images $\mathcal{S} = \{S_1, ..., S_N\}$ that appear in the
pattern.  It jointly optimizes the parameters of a similarity transform (i.e.,
translation, rotation and uniform scale) for each source element as well as
their visibility layer ordering so that when the transformed elements are rendered in
back-to-front order they reproduce the target pattern.  That is,
\begin{equation}
  %\text{DC}(\mathcal{S}, T) = \{(S_i, \Theta_{S_i}, \Lambda_{S_i}) | \forall S_i \in \mathcal{S} \},
  \text{DC}(\mathcal{S}, T) = \{(S_1, \Theta_{S_1}, \Lambda_{S_1}), ...,  (S_N, \Theta_{S_N}, \Lambda_{S_N})\},
\end{equation}
% \sharon{
% \begin{equation}
%   %\text{DC}(\mathcal{S}, T) = \{(S_i, \Theta_{S_i}, \Lambda_{S_i}) | \forall S_i \in \mathcal{S} \},
%   \text{DC}(\mathcal{S}, T) = \{(\Theta_{S_1}, \Lambda_{S_1}), ...,  (\Theta_{S_N}, \Lambda_{S_N})\},
% \end{equation}
% }
where $\Theta_{S_i}$ is the transform that maps $S_i$ to it's
placement in $T$, and $\Lambda_{S_i}$ is the layer z-ordering (larger
z's are in front of lower z's) for $S_i$ with respect to the other
elements in $\mathcal{S}$ after they have been transformed by their
respective $\Theta$'s.
%
We refer to the resulting set of layering placement tuples as
$\mathcal{S}^* = \{(S_i, \Theta_{S_i}, \Lambda_{S_i})\}^N_{i=1}$
% \sharon{By applying the corresponding transformations, we can define a resulting set of layering placement tuples as $\mathcal{S}^* = \{(\Theta_{S_i}(S_i), \Lambda_{S_i})\}^N_{i=1}$}
%
%\maneesh{Maybe define the
%  compositing function and Mvis later when we need them.}
%We can also define a compositing function $\mathcal{C}(\mathcal{S}^*)$
%that composites the all source elements in $\mathcal{S}$ after they
%have been transformed by their respective $\Theta$'s and layered using
%their respective $\Lambda$'s.
%
%Similarly we can
%
With this information we can for example,
compute a binary mask $M^\text{vis}_{S_i}(S_i,
\mathcal{S}^*)$ 
% \sharon{$M^\text{vis}(S_i,
% \mathcal{S}^*)$} 
of the visible parts of $S_i$ with respect to the
other elements in $\mathcal{S}$ after they have all been transformed
by their respective $\Theta$'s and layered using their respective
$\Lambda$'s.
%their respective $\Lambda$'s.
%With this information we can, for example, generate the composite
%image $\mathcal{I}^\text{cmp}(\Theta(\mathcal{S}))$ of the set of
%source elements $\mathcal{S}$ after they have all been placed in $T$
%according to their $\Theta$'s and composited using their $\Lambda$'s.
%Similarly we can build a binary mask
%$M^\text{vis}_i(\Theta_i(S_i))$ of the visible parts of $S_i$ with
%respect to the other elements in $\mathcal{S}$ after they have all
%been placed and composited.
%With this information we can, for example, compute a binary mask
%$M^\text{vis}_i(\Theta_i(S_i))$ of the visible parts of $S_i$ with
%respect to the other elements in $\mathcal{S}$ after they have all
%been placed in $T$ according to their $\Theta$'s and composited using their
%$\Lambda$'s.

\vspace{0.5em}
\noindent
{\bf \em Our extensions.} 
To apply differential compositing to the context of tracking objects
in motion graphics video, we have extended the optimization to
explicitly compute an affine transformation (i.e., translation,
rotation, non-uniform scale and shear) $\Theta_{S_i}$ rather than a
similarity transform. Specifically we add transformation parameters
for x-scale, y-scale, x-shear and y-shear as independent variables in
the optimization.
%
%In addition, differential compositing was originally used to decompose
%graphic patterns where each source element could appear lots of times
%in the target image. So, they used an overlap loss to penalize the
%optimizer

We also define 
%We also use the layered placement information $\mathcal{S}^*$ to define
a new loss function $\mathcal{L}_\text{vis}$
that compares the pixel match between
source element $S_i$ and the target image $T$, while properly
accounting for visibility, using the layering placement information $\mathcal{S}^*$,
%after being transformed by $\Theta_i$ while
%accounting for occlusions given by $\Lambda_i$, as
\begin{equation}
  \mathcal{L}_\text{vis}(S_i,T,\mathcal{S}^*) = \mathcal{L}_\text{int}(S_i,T,\mathcal{S}^*) + \mathcal{L}_\text{xor}(S_i,T,\mathcal{S}^*).
\end{equation}
The first term $\mathcal{L}_\text{int}$ measures the $l^2-norm$ color difference between the
visible pixels of $S_i$ and corresponding pixels in $T$ wherever they intersect in the target space. Specifically,
\begin{equation}
  \mathcal{L}_\text{int} = ||M^\text{int} \otimes (\Theta_{S_i}(S_i) - T)||_2,
  \label{eq:Lint}
\end{equation}
% \sharon{do we need the following text clarification before the equation?} 
where $\otimes$ denotes pixel-wise multiplication, and
$M^\text{int}$ is a binary mask representing the pixels of $\Theta_{S_i}(S_i)$ that
are both visible in the target space $M^\text{vis}_{S_i}(S_i, \mathcal{S}^*)$, and that are
also within $T$. That is,
\begin{equation}
  %  M^\text{int} = M^\text{vis}_{S_i}(\Theta_{S_i}(S_i)) \cap T.
  M^\text{int} = M^\text{vis}_{S_i}(S_i, \mathcal{S}^*) \cap T.
    \label{eq:Mint}
\end{equation}
The second term $\mathcal{L}_\text{xor}$ penalizes the areas where
$\Theta_{S_i}(S_i)$ and $T$ do not align -- i.e., pixels {\em only} occupied by
$\Theta_{S_i}(S_i)$ or {\em only} by $T$, as
\begin{equation}
  %  \mathcal{L}_\text{xor} = \frac{|M^\text{vis}_{S_i}(\Theta_{S_i}(S_i)) \oplus T|}{|M^\text{vis}_{S_i}(\Theta_{S_i}(S_i)) \cup T |}.
  \mathcal{L}_\text{xor} = \frac{|M^\text{vis}_{S_i}(S_i,\mathcal{S}^*) \oplus T|}{|M^\text{vis}_{S_i}(S_i, \mathcal{S}^*) \cup T |}.
    \label{eq:Lxor}
\end{equation}
Here, $\oplus$ denotes the pixel-wise XOR operator and the ratio
computes the mismatched area between $\Theta_i(S_i)$ and $T$ as a
percentage of the total area covered by their union.
%
\maneesh{Update next sentence to talk about taking a subset of elements for T as well as for S.}
We can further compute
$\mathcal{L}_\text{vis}(\widetilde{\mathcal{S}},T,\mathcal{S}^*)$
where $\widetilde{\mathcal{S}} \subseteq \mathcal{S}$ is a subset of
the source elements, rather than a single source element.
\maneesh{Maybe move rest of paragraph to appendix and write out equations fully. Need to include case where T is a set of regions.}
For this we
first define a compositing function
$\mathcal{C}(\widetilde{\mathcal{S}}, \mathcal{S}^*)$ that composites
the source elements in $\widetilde{\mathcal{S}}$ after they have been
transformed by their respective $\Theta$'s and layered using their
respective $\Lambda$'s.  Then to compute
$\mathcal{L}_\text{vis}(\widetilde{\mathcal{S}},T,\mathcal{S}^*)$ we
replace $\Theta_{S_i}(S_i)$ in Equation~\ref{eq:Lint} with
$\mathcal{C}(\widetilde{\mathcal{S}}, \mathcal{S}^*)$, and we replace
$M^\text{vis}_{S_i}(S_i,\mathcal{S}^*)$ in Equations~\ref{eq:Mint}
and~\ref{eq:Lxor} with $\bigcup_{S_i\in \widetilde{\mathcal{S}}}
M^\text{vis}_{S_i}(S_i,\mathcal{S}^*)$. \sharon{Can we just describe everything in terms of a subset and mention that a subset can be a single source element?}


==> induction.tex <==
\section{Program induction}\label{sec:induction}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{skeleton_figs/system.png}
    \caption{System overview}
    \label{fig:system}
\end{figure*}

Our program induction pipeline has three main parts
(Figure~\ref{fig:system}).  The first module performs \textit{region
  extraction} on every frame of the input video. The per-frame region
information is then passed to an \textit{identification} module which
assigns a unique label to regions corresponding to the same
object. This module also extracts a canonical appearance for each
object. This resulting information is passed to the final
\textit{motion recovery} module, which determines the affine
transformation applied to the object appearance at every frame.
% \maneesh{I think ``tracking'' is a term for the whole pipeline -- or
%   at least the part that computes frame to frame motions seems to be
%   the ``tracking'' component. I might change the names to (1) Region
%   Extraction, (2) Shape/Region Matching (or Shape/Region
%   Identification) and (3) Motion Tracking (or Motion/Warp
%   Recovery). Also we should look at related work to see if the
%   Tracking literature already names thees components.}

% The resulting program can be rendered to a browser with SVG or loaded
% into other editing software such as After Effects and Blender. In
% Section~\ref{sec:apps}, we also demonstrate some automated video
% editing tasks by applying certain functions to the \program itself and
% output a modified \program. \maneesh{At this point readers should know
% that we will show applications of the resulting SVGs later. I think we can remove it from here.}

\maneesh{May eventually want to move assumptions before describing three stage pipeline.}
The space of motion graphics videos covers a large variety of visual
effects, motions and transitions, some of which are hard to reason
through vis-\'{a}-vis object tracking. \maneesh{Not clear what ``hard to reason through'' means. It will be stronger
  to say that we focus on a very common form of motion graphics (perhaps most common if we can quantify this loosely but in a reasonable way).}
Fortunately, a large class of
motion graphics is characterized by design principles that we now
summarize with two assumptions \maneesh{Not sure these assumptions are related to ``design principles''. One way we can approach this is to say that there are a set of design principles used by a large class of motion graphics videos -- each principle should be motivated by what it helps with in terms of communicating to viewers. The clear boundaries bullet does this. Once we have stated the design principles we can say what we focus on motion graphics that are designed according to them. Alternatively we can say that we make certain (simplifying) assumptions -- this may be the case when there isn't a clear design principle.}: 
% To concretely define a  we introduce a set of
% assumptions on the objects and motions in our input videos.
% \maneesh{I think the reasoning needs to be a bit more explicit in this paragraph. Motion graphics vary a lot, but a large class of them fit a few assumptions... Would be even stronger if we could explain why they fit these assumptions. My sense is that there is a large class of motion graphics videos that are 2D affine motions of solid colors, gradients and patterns formed from a small palette of colors. Can we find books on motion graphics that say this or something similar. Can we base this on examples?}

\sharon{Find citations in motion graphics books below.}
\begin{enumerate}
    \item \textbf{Clear visual boundaries.} In order to improve perception and legibility, many motion graphics videos have distinct separation between foreground and background, as well as between objects. Many advertisements, for example, will have a solid-colored background and foreground objects and text that is well-contrasted against the background. \maneesh{I could imagine objects with clear boundaries but that are not solid colored.}
      % New objects frequently
      % appear and disappear at various points in motion graphics
      % videos. In order to avoid burdening a user with the task of
      % scrubbing through an entire video and indicating each unique
      % object that appears, we opt to automatically extract unique
      % objects. To reliably do so, we assume that all objects are
      % bounded by a clear visual border and have no internal borders.
      % \maneesh{I wouldn't worry about explaining why it would be herd for a user to specify boundaries. I think each of these bullets should explain why videos tend to follow these assumptions -- visible boundaries allow viewers to visually/perceptually separate foreground objects from one another and from the background.}

      % \item \textbf{Uniform background.} A large subset of motion graphics videos use uniform background colors for the same reasons that they 
      % Since the video
      % background typically will not adhere to an affine motion model,
      % we perform foreground-background segmentation and only extract
      % regions from the foreground. \todo.
      % \maneesh{Why won't background adhere to affine motion? I think often it will. I think we should think about this limitation and whether we can remove it or at least partially remove it. What we need is a good background segmenter or matte extractor. Seems like there should be a few things to try here.}
    
    \item \textbf{Affine motion model.} Affine transformations describe essential motions like scale, rotation and translation. For the sake of clarity and minimizing visual distractions, many objects in motion graphics videos will adhere to these basic movements~\cite{}. to introduce objects into a frame, motion designers often use transitions like fades \sharon{take out? we don't model opacity}, \maneesh{We should talk about these transitions separately -- not as part of the motion model. Should list the most common transitions and say up front if we don't handle any of them.} slide ins, and bounces. Animation principles such as squash-and-stretch or slow-in and slow-out also appear commonly. We can describe each of these events with affine transforms as well.  \maneesh{This one is not really written like a design principle because it doesn't explain why affine motions are good for viewers -- how they aid perception/cognition.}
      % We assume an affine model on
      % the object's appearance. This is consistent with the basic
      % features of video timeline editors in programs such as Adobe
      % After Effects~\cite{} and \todo.
      % \maneesh{I think it would be stronger motivation to explain why an affine model still allows a wide variety of videos and why so many videos fit this assumption. Also it is not clear that After Effects limits to affine motions -- it might allow homographics -- I'm not sure if non-uniform shears enable homographies. }
\end{enumerate}

% The goal of our pipeline is to recover all independent objects and
% their motions from a given input video. There are three main parts to this pipeline. First, we identify
% all object regions in a \textit{region extraction} step. Next, we perform \textit{object identification} and assign a label to each unique object in the video. We label any pixel in an object region that is covered by the object of that label. This results in a set of object masks sequences.
% After identification, we then determine the motion parameters of all the objects in a \textit{motion recovery} module.
% \maneesh{Previous paragraph is redundant with current first paragraph of section. Should only state this once.}
% \maneesh{This paragraph is
%   really part of the system overview. I think it should be combined
%   with what we have there. Leading with the goal is good! We should
%   consistently use the names for each of the pieces of pipeline --
%   region extraction, shape matching, motion recovery -- or some such.}

%% Motion file extraction
 % Vocabulary
 % - Object := one unique layer in the representation containing a template and set of parameter curves
 % - Templates := canonical object appearances
 % - Shape := a region in a frame
 % - Identified shape := a shape region which has been assigned to an object
 % - Unidentified shape := a shape region which has not been assigned to an object

% \maneesh{The subsections here seem like they should be subsections of the section 3. I would call section 3 Method but keep the text of the system overview as the first part of the section, then put the subsections here after that.}

In the following sections we describe how we determine the mappings. First, we give a brief overview of the differentiable compositing method by Reddy~\etal~\cite{}, which is an integral component to our pipeline. Next, we describe in detail how each of the three modules in our system works.

\input{diff_comp.tex}
\input{pipeline_i.tex}
\input{pipeline_ii.tex}
\input{pipeline_iii.tex}

% LocalWords:  vis


==> intro.tex <==
\section{Introduction}
\label{sec:intro}

%\begin{figure*}[t]
%    \centering
%    \includegraphics[width=\textwidth]{skeleton_figs/teaser.png}
%    \caption{Teasure figure.}
%    \label{fig:teaser}
%\end{figure*}

%\maneesh{Outline: \\
%  1. Why motion graphics are an important domain (also define motion graphics).\\
%  2. Why a program is a useful representation to recover (can also suggest that this has been done in prior work for other visual domains -- visualization (revision paper and others), L-systems (), etc.\\
%  3. In this paper we ... Our key insight is ... \\
%  4. Summary of things we can do with the program representation (the apps) \\
%  5. Contribution bullet points.
%}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Version 2 (12/23/22)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% DRAFT START
Programs have proven to be incredibly useful in many areas of computer
graphics. The structure and repetition found naturally in our
surroundings combined with the symbolic reasoning that humans use to
describe objects make programs particularly useful in representing
visual content. For instance, biologists use L-systems to model plant
structures~\cite{prusinkiewicz_lindenmayer_1996}; digital artists use shader graphs to generate
materials and textures~\cite{Cook1984}; visualization tools use grammars to
create charts and graphs~\cite{2017-vega-lite}; and SVG is a widely adopted 
declarative program format 
for vector graphics~\cite{svg2}. 
%\maneesh{Let's talk about whether
%we should use the word ``repetition''. Also let's start to fill in the citations.}
% To produce a single image in software like Blender~\cite{}, for
% example, an artist may have interfaced with multiple
% programs--L-systems to model the growth of trees and other
% vegetation, urban parametric modeling for architecture and city
% layouts, and shader graphs to generate various textures and
% materials. Even beyond 3D modeling, programs have been used in
% visualization work~\cite{}, vector graphics~\cite{}, and video
% editing~\cite{}. \maneesh{We might be going a bit too far away from
% motion by talking about scene generation in Blender. I might tighten
% by talking more directly about the programming tools used to create
% a variety of different types of content. L-systems for vegetation,
% SVG for vector graphics (end with that one), grammars for for charts
% and graphs, shader graphs for materials and textures. Put a citation
% for each one.}

There are several benefits to representing visual content with a
program, rather than working directly in the output space of pixels,
images and frames.
%There are several benefits to working with a program representation
%rather than directly in the output space.
For one, programs function at a higher level of abstraction than
pixels, thus allowing for more meaningful concepts to be defined.
\maneesh{avoid passive voice. -- For one, programming languages often
  provide meaningful abstractions and concepts (e.g. API primitives)
  that operate at a higher level than pixels and often correspond
  better to the ways that humans think about the underlying
  content. -- will need a bit of work to integrate this sentence if we
  keep it into the paragraph.}  \sharon{Tune the following example.}
It is much easier to identify a region in an image as the letter `A'
than a set of black pixels. If we extend this single image into
consecutive video frames, we can continue to use the single identifier
`A' even as the number of pixels grows quickly.  Another benefit of
programs is that they allows us to describe outputs with meaningful
input parameters. Basic shapes, for example, can be specified by a few
controls such as radius, width and height. The same shapes can then be
quickly edited by toggling these few parameters.
% For one, program
% representations can be much more compact than the program
% output. Additionally, programs take advantage of repetitive processes
% by abstracting them into higher level functions. For a domain like
% video, which requires users to keep track of information across time,
% program representations can greatly reduce the manual work needed to
% generate a single change.
% \maneesh{We should talk about the benefits in priority order. I might
%   contrast programs as a higher-level (more abstract/meaningful) representation
%   than images/video which are a pixel-level representation (objects can be described using shapes rather than pixels). I think
%   the biggest benefit of the program representation is this abstraction
%   to a higher level than pixels. I worry a bit about introducing the idea
%   of repetitions as something that is handled in programs, as our programs
%   are not really designed to handle repetition at the moment -- we don't
%   really have loops -- though we might if we interpolate the motion paths -- but
%   I think think that will be core to this work. I might avoid talking about
%   repetition. The other advantage of programs is that they include meaningful control parameters
%   that can be manipulated to adapt and change the output. Compactness I think is a less important
%   benefit.}

% \maneesh{I think we can directly turn to motion graphics at this point and cover the idea of program induction in the context of
%   motion graphics later. We do want to say at that point that the vast majority of motion graphics are only available as sequences of video frames
% and without access to a program based representation, manipulating the output is prohibitively difficult.}
% Despite the advantages of working with a program representation, it is
% not usually the case that we have access to a programmatic form of
% visual media. This motivates the task of visual \textit{program
%   induction}, which seeks to produce that program. Program induction
% has been studied extensively in both visual and non-visual domains. In
% this work, we propose to study program induction for \textit{motion
%   graphics}, a category of visual media that is particularly suitable
% for programmatic representations due to its structure and creation
% process. 

One domain of visual media which fits neatly into the programming
paradigm is the space of \textit{motion graphics}.  \dr{This topic
  sentence might make some readers think that motion graphics have
  already been explored in the context of programs, whereas we want to
  claim this framing as our novel contribution.} \maneesh{Agree. I think we want to rework the sentence
  -- maybe start by saying what motion graphics are as in next sentences but say right away that the most common format it video frames of pixels and so creating variations is difficult.}
% One domain of visual media that heavily relies on working at the object-level is \textit{motion graphics}.
Motion graphics are a broad category of animated graphic design that
appear in film sequences, web design, digital advertising and many other media (Figure~\ref{fig:teaser}).
% \maneesh{maybe move advertising to the
%   end of list and be more specific about the kinds of sequences --
%   title sequences in film, -- I'm not sure where exactly they appear
%   in documentaries or in web design. We should point to the teaser as
%   that will have an example of a motion graphic.}  
At their core, motion graphics are essentially animated graphic
design, placing images, vector shapes and typography together with
choreographed motions. In this work, we focus on a videos that
specifically uses affine motions on uniformly colored objects. While
this space of videos is not comprehensive of all motion graphics, it
characterizes a large subset of work produced by motion
designers~\cite{}. \maneesh{What citation can we use here? Can we quantify the size of this subset in some way? Point sites like dribble and others perhaps?}
% \maneesh{We may need to limit to solid colored/gradient/minimal
%   texture objects, affine motion, etc. and say something about this
%   still being a very large class of motion graphics video. We want to
%   make sure we are setting reviewer expectations about the work
%   appropriately. Not sure there is always a strong narrative. For
%   example, animated logos are a large class of motion graphics. }
% Though they often have natural video elements, motion graphics artists
% will typically apply principles from traditional hand-drawn animation
% to how they design these videos; as such, many objects in motion
% graphics will undergo highly stylized motions and deformations.
% \maneesh{I would avoid talking about natural video elements and traditional hand-drawn motion styles (e.g. squash and stretch) as we currently don't handle these things.I would try to focus the paragraph primarily on the kinds of motion graphics we do handle.}

Despite the popularity of using motion graphics in digital media,
these videos are presented to the general viewer only as frames of
pixels. Though the original video may have been created with
individual objects undergoing independent motions, this information is
not explicitly accessible in its video form and thus editing these
videos becomes extremely difficult. Advertising companies may want to
swap out objects, replace text, or retime the video to various audio
tracks to generate personalized content.  \dr{I'd suggest coming up
  with a different motivating use case, because ``advertising
  companies'' would presumably have access to the source files used to
  create their motion graphics in the first place.} \maneesh{Agree. I think personalizing
or use-cases where lots of variations have to be generated could be compelling.}
A video may also
need to adapt to an unknown aspect ratio to fit in a particular
window. Given a representation of the video that describes unique
shapes and their motions independently, these tasks boil down to an
adjustment of some object-level parameters. Otherwise, the same
adjustments may require manually editing the video frame by frame.

% Though there is an entire professional industry centered around motion
% graphics and motion designers, today sites like Biteable~\cite{} and
% LottieFiles~\cite{} allow non-designers to quickly put together motion
% graphics from templates and customizable assets.
% \maneesh{I think the last part of the last sentence about Biteable and LottieFiles is a little
%   distracting because it suggests that our work may not be necessary. Rather we want to end this paragraph
%   by stating the basic issue -- most common representation of motion graphics is video frames making them
%   difficult to manipulate. We should also introduce the types of manipulations one might want to do -- change
% the objects, the text, translation, personalization, aspect ratio, retiming etc. I think it is important to state them upfront as they motivate our work a lot.}

In this work, we present a system which converts a motion graphics
video into an SVG~\cite{svg2} program. Our {\em program induction} pipeline
tracks unique objects through each frame and determines their affine
parameters using a differentiable compositing optimization
method~\cite{Reddy2020}. The resulting program can be loaded into an SVG
renderer (\eg a Web browser) or other editing software (\eg Adobe
After Effects~\cite{christiansen2013adobe}) and manipulated to generate variations of the
original video. We also introduce a set of semi-automated {\em program
transformations} that allow users to apply specific adjustments to the
input video via our recovered programs. Specifically, we demonstrate
how to change the objects, timing, motion, physical appearance and
aspect ratio of the input video in a content-aware manner. \sharon{Our
  results show that...}

%% \maneesh{I think we need a paragraph here saying that ... in this work
%%   we convert motion graphics video into higher-level motion programs
%%   (SVG + SMIL).  Our approach is ... (one sentence giving high level
%%   of our approach to program induction.)  Users can load the resulting
%%   programs into any SVG renderer (including a Web browser), to
%%   regenerate the input video or use an SVG editor to change its
%%   content. (Not sure if previous sentence should be said so strongly
%%   maybe it needs to be toned down.)  We also introduce a set of
%%   semi-automated program transformation tools that let users
%%   manipulate the resulting motion programs and generate variations of
%%   the input video.  Specifically we demonstrate how the program
%%   transformations can be used to easily change the timing, motion
%%   paths, objects, text, aspect ratio, (more here) to personalize,
%%   translate, (higher level goals of manipulation)... the input
%%   video. (Need to also explain that program transformations can be
%%   applied to any SVG program and not just those output by our
%%   induction system.}

%% \maneesh{May need a last paragraph describing an overview of the results. That may also be incorporated into the previous paragraph.}

% Like traditional video editing and 3D animation, motion graphics is
% usually made by specifying how different objects deform and move as a
% function over time. These deformation parameters may include scale,
% rotation, translation and other non-affine parameters, and they are
% generally represented using some polynomial spline basis. This
% object-centric structure is reminiscent of a program: it disentangles
% the lifetime of an object in the video into two inputs, a canonical
% appearance and a set of functions parameterized by time, and it also
% allows independent objects to be treated separately. As a result,
% users only need to adjust a limited set of controls to adjust objects
% in the video, as opposed to making changes at the pixel and frame
% level.
% \maneesh{I think this paragraph may come later -- it is too much detail
%   about our program representation for the intro. It also is definitely a
% declarative program. I wouldn't call it reminiscent of a program.}

% Our programs describe both the appearance and motion of the objects within the video, and we demonstrate how these programs allow various manual editing tasks to be automated. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Version 1 (12/19/22)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% High-level notes
% - Concrete examples of motion graphics that people will immediately recognize (ads, banners etc.), also include in teaser
% Focus less on how they are created--highlight their output as video representation.
% Flip order? Why we want programs, then motiongrphics vs. motion graphics then why programs
% We experience motion graphics as video, but it is more structured than regular/natural video, lends to a programmatic structure. Add examples of this (what types of aspects would represntable w/ programs?)
% Programs expose crtain parameters that might be more useful, etc.
% Provide a more detailed decription of what is happening in the video
% General pattern in visual computing for describing content
% Sometimes it is ambiguous what the langauge to describe that program should be, but we still want to describe it that way 
% LCD = pixels
% Nail vs. hammer style paper? Nail approach might set high expectations for handling all motion graphics
% Get precise language around SVG + SMIL (include a citation)
% "Subset" of what is expressed in a particular exiting library, helpful to anchor but not necessarily completely compatible--make use of the SVG output we have
% 2D graphics, SVG inference -- use Eurographics preprint on neurosymbolic programming for related work section

%%% DRAFT START
% From object tracking to realistic character animation, describing motion has been a longstanding problem in computer vision and computer graphics. Yet motion in digital media is much more ubiquitous than raw video footage or 3D animation. \textit{Motion graphics} is a broad category of animated graphic design that appears in advertising, documentaries, film sequences, web design and many other media. At its core, motion graphics is essentially animated graphic design, often placing images, vector shapes and typography together to create a narrative. Though they often have natural video elements, motion graphics artists will typically apply principles from traditional hand-drawn animation to how they design these videos; as such, many objects in motion graphics will undergo highly stylized motions and deformations. Though there is an entire professional industry centered around motion graphics and motion designers, today sites like Biteable~\cite{} and LottieFiles~\cite{} allow non-designers to quickly put together motion graphics from templates and customizable assets.

% Like traditional video editing and 3D animation, motion graphics is usually made with software like Blender~\cite{} or Adobe After Effects~\cite{}. These editors generally have a video timeline interface in which users can, at the most basic level, create layers that specify some motion and deformation parameters to an object or group of objects. These deformation parameters may include scale, rotation, translation and other non-affine parameters, and they are generally represented using some polynomial spline basis. This object layer structure is reminiscent of a program: it disentangles the lifetime of an object in the video into two inputs, a canonical appearance and a set of functions parameterized by time, and it also allows independent objects to be treated separately. As a result, users only need to adjust a limited set of controls to adjust objects in the video, as opposed to making changes at the pixel and frame level.

% Visual programs have been used in a variety of other domains to help facilitate content creation. \sharon{Sentence including L-systems in biology, 3D shape generation, visualization tools.} There are several benefits to working with a program representation rather than directly in the output space. For one, program representations can be much more compact than the program output. Additionally, programs take advantage of repetitive processes by abstracting them into higher level functions. For a domain like video, which requires users to keep track of information across time, program representations can greatly reduce the manual work needed to generate a single change.

% Despite the advantages of working with a program representation, it is not usually the case that we have access to a program form of visual media. In this work, we introduce a system to recover \program s for motion graphics videos. Though many motion tracking systems exist for natural video, motion graphics videos have certain animated characteristics which preclude the direct application of such systems and require additional careful treatment. By exposing this program, we allow users to use existing videos as starting templates for creating new videos. Our programs describe both the appearance and motion of the objects within the video, and we demonstrate how these programs allow various manual editing tasks to be automated. 

In summary, our contributions are:

\begin{enumerate}
    \item A system which recovers an SVG+SMIL motion program for an input motion graphics video; this program can then be directly edited and re-rendered to generate new videos. % Emphasis on resulting program
    \item A demonstration of various fully and semi-automated video editing applications using the resulting program files. \maneesh{Let's talk about this as ``program transformation''}
\end{enumerate}
% Reminder: contributions are evaluated by the paper

% Hinting at first step of extracting a program that goes beyond the video timeline--do we need to mention this that much?

\sharon{Note about code and demos.}

\maneesh{Teaser should maybe show an input video, the program presentation and then maybe applications.}



% LocalWords:  shader SVG Biteable LottieFiles customizable retiming
% LocalWords:  personalization SMIL renderer centric spatiotemporal
% LocalWords:  retime


==> method.tex <==
\section{Method}
\label{sec:method}
% Every time we decribe a new component in the system, introduce the context

The goal of our pipeline is to recover all independent objects and
their motions from a given input video. To do so, we first identify
all foreground regions. After identifying which regions correspond to
which objects, we can determine the scale, rotation, skew and
translation of every object at each frame.  \maneesh{This paragraph is
  really part of the system overview. I think it should be combined
  with what we have there. Leading with the goal is good! We should
  consistently use the names for each of the pieces of pipeline --
  region extraction, shape matching, motion recovery -- or some such.}

%% Motion file extraction
 % Vocabulary
 % - Object := one unique layer in the representation containing a template and set of parameter curves
 % - Templates := canonical object appearances
 % - Shape := a region in a frame
 % - Identified shape := a shape region which has been assigned to an object
 % - Unidentified shape := a shape region which has not been assigned to an object

\maneesh{The subsections here seem like they should be subsections of the section 3. I would call section 3 Method but keep the text of the system overview as the first part of the section, then put the subsections here after that.}

\subsection{Region extraction}

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{skeleton_figs/region_extraction.png}
    \caption{Region extraction.}
    \label{fig:region_extraction}
\end{figure}

Our region extraction method is an edge-based segmentation
approach. Given a frame $F$ of the input motion graphics video, we first convert it to LAB colorspace and
apply a Canny edge detector~\cite{} on the luminance channel to
generate a binary edge image. Then, we obtain a set of foreground
regions $\mathcal{R} = \{ R_1, \ldots, R_N \}$ using the trapped-ball
segmentation method of Zhang~\etal~\cite{}. In the final
\program, every pixel in a region will be covered by an object; all
other pixels are considered background. 
\maneesh{I might use lowercase $f$ for frames.}
\maneesh{I would avoid future tense and the word ``will'' as it can be confusing as to when something ``will'' happen. Last sentence is
also confusing because it is unclear what an ``object'' is.}

\subsection{Object tracking}
% Why is tracking hard?
% We do not follow the detection-based or detection-free tracking paradigm.
% We do not have a trained model to do detection, nor can we ask the user to manually specify every instance of a new object.
Once we have determined a set of regions for every input frame, we proceed
to assign object identifiers to frame regions in chronological
order.
\maneesh{What is an ``object identifier'' and more importantly why do we need to assign one to each region.}
At the first frame, each region is automatically assumed to be
a unique object. This gives us an initial set of existing objects and
their appearances. The regions in the next frame will then need to be
assigned either (1) an object identifier from the first frame or (2) a
new unique object identifier. Since labeling new regions with
identifiers depends on the objects we have already tracked, we also
keep an \textbf{object bank} \maneesh{alt: object list} that stores the most recent centroid,
bounding box, mask and time that each previously identified object
appeared.

Assume that we have tracked some objects from frame $1, \ldots, t -
1$. Given the next frame $F_t$ and its regions $\mathcal{R}_t = \{
R_1, \ldots, R_N \}$, our goal is to compute a mapping between
$\mathcal{R}_t$ and the set of object shapes \maneesh{what is a
  ``shape'' and how is it different from a ``region''?} in $F_{t -
  1}$, which we call $\mathcal{S}_{t - 1} = \{ S_1, \ldots, S_M
\}$. The mapping determines how we assign identifiers to each $R_j$,
\eg if $S_1$ is matched to $R_1$, then we assign the identifier of
$S_1$ to $R_1$.
\maneesh{I wonder if we should call the ``mapping'' the ``assignment mapping''. Should also check if there is terminology in the tracking literature about this.}
Note however, that it is not necessarily case that a
single shape at time $t - 1$ should be matched to a single region at
time $t$.  \maneesh{alt: Note however that the mappings between shapes and regions is not always one-to-one. (May need to introduce all the cases we handle here -- many-to-one and one-to-many and explain why we don't need many-to-many.}

We model this mapping problem with a bipartite graph $B =
(\mathcal{S}_{t - 1}, \mathcal{R}_t)$.  \maneesh{To compute the
  assignment mapping we build a bipartite graph ... (I think the term
  ``mapping problem'' is confusing as we haven't really stated what
  the problem is. The way the mapping is defined above suggests that
  it is the final chosen mapping between shapes and regions and that
  correspondences as described below are hypotheses for the true
  mappings. So the problem is to pick the best mapping amongst the
  hypotheses.}  Edges in the graph $e = (S_i, R_j)$ indicate a
possible correspondence between a shape in the previous frame $S_i$
and a region in the current frame $R_j$ (for brevity, we drop
``previous" and ``current" and it is assumed that ``shape" refers to
the previous frame and ``region" refers to the current frame).
\maneesh{I think we should explain the parenthetical statement up
  front in this subsection and remove the parens.}  These
correspondences will determine which object identifiers are propagated
to which regions. \maneesh{The correspondences don't directly
  determine this. We use the correspondences as hypotheses for the
  final mappings and the goal is to pick the ``best'' hypothesis.}
There are two stages to this mapping problem; We first coarsely match
shapes to regions using appearance and optical flow cues
(Section\,\ref{sec:coarse_match}) and then, we optimize the affine
parameters of shapes against their target regions (and vice versa) to
determine our final mapping (Section\,\ref{sec:fine_match}).

\maneesh{I was assuming the next two subsubsections would describe the
  coarse matching and then the optimization. Headings suggest they
  describe something else. We should make the headings consistent. I might also change ``optimization'' to fine matching.}


\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{skeleton_figs/coarse_mapping.png}
    \caption{Coarse mappings.}
    \label{fig:coarse_mapping}
\end{figure}

\subsubsection{Limiting the search space}
\label{sec:coarse_match}
Ultimately, we want to determine the exact position and location of
each shape from frame $F_{t - 1}$ in frame $F_t$. This will be done by
applying the differentiable compositing framework~\cite{} on
shape-region correspondences, as described in the follow
Section~\ref{fine_match}. However, this process requires a good
initialization of the parameters being optimized, \ie we must make a
good initial guess at the affine transformation to apply to an element
in order to converge accurately to its target appearance.
\maneesh{This paragraph seems out of place as it seems like a
  higher-level abstract of the approach. Also we are in the
  shape/region mapping section, so we want to focus on the specific
  problem here of computing correspondence hypotheses.}

Initially, we assume a complete bipartite graph $B$. To provide the
subsequent optimization with a good initialization, we first reduce
the search space by deleting edges of $B$ that represent improbable
correspondences.
\maneesh{We should explain the general idea (e.g. the features we will be considering) before presenting the equation. Not sure
how a weight allows us to delete edges.}
We accomplish this by assigning a weight
\begin{equation}
    w(S_i, R_j) = \overrightarrow{f}(S_i, R_j) * \overleftarrow{f}(S_i, R_j) * d_{rgb}(S_i, R_j) * d_c(S_i, R_j),
\end{equation}
to each edge. This weight is the product of four score functions. The first two are the \textit{forward intersection} and \textit{backward intersection} scores, defined as
\begin{equation}
    \overrightarrow{f}(A, B) = |\overrightarrow{\mathcal{F}}_{t - 1}(A) \cap B|
\end{equation}
and
\begin{equation}
    \overrightarrow{\mathcal{F}}(A, B) = |A \cap \overleftarrow{\mathcal{F}}_t(B)|,
\end{equation}
respectively. Here, $\overrightarrow{\mathcal{F}}_{t - 1}$ and
$\overleftarrow{\mathcal{F}_t}$ denote the optical flow from frame
$F_{t - 1}$ to frame $F_t$ and vice versa, respectively.  \maneesh{I
  think we want to first explain why flow in the forward direction
  with the intersection score can be used as a hypothesis. Then
  explain why backwards flow is also useful, then talk about
  appearance score. Build these up explain why each score is useful
  and then give the form of the score as an equation and finally
  combine all the scores into a weight.}  Essentially, these scores
compute how much shape $S_i$ intersects with region $R_j$ according to
an optical flow prediction, which we compute using a RAFT
model~\cite{} pretrained on the Sintel~\cite{} dataset. \maneesh{I
  think we should clarify that RAFT is just the optical flow
  computation, not the score computation -- right?}

We also compute a color similarity score
\begin{equation}
    d_{rgb}(S_i, R_j) = 1.0 - \text{Hellinger}(hist_{LAB}(S_i), hist_{LAB}(R_j))
\end{equation}
that measures the similarity between LAB colorspace histograms of
$S_i$ and $R_j$. Here we use the Hellinger distance~\cite{} to compute
that similarity.
\maneesh{$d$ implies a distance, but we are actually computing a similarity I think. We should
rename our variable for appearance -- maybe to $a$. Also I would remove the work Hellinger from the equation and instead maybe use $d_{Hel}$ or just $d$ and explain that it is the Hellinger distance.}
Finally, we also compute a contour feature score
\begin{equation}
    d_c(S_i, R_j) = 1.0 - | \langle \text{efd}(S_i), \text{efd}(R_j) \rangle |
\end{equation}
that first computes elliptic Fourier descriptors~\cite{} for the
contours of two shapes and then measures the absolute cosine
similarity between them. \maneesh{Need to say how many terms we keep in the descriptor.}

\subsubsection{Fine mappings}\label{sec:fine_match}
The result of the previous stage is a weighted undirected bipartite
graph $B$. In this stage, we want to determine a set of
\textit{directed mappings} between shapes and regions.
\maneesh{We haven't explained how we go from weights to an undirected graph. Specifically we haven't said anything about dropping edges from the complete graph.}
Mappings are of
the form $S \rightarrow R$ or $S \leftarrow R$, where $S \subseteq
\mathcal{S}_{t - 1}$, $R \subseteq \mathcal{R}_t$ and the arrow
indicates a forward or backward direction. We identify five different
types of valid mappings: 

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{skeleton_figs/cases.png}
    \caption{Label propagation cases.}
    \label{fig:cases}
\end{figure*}

\begin{enumerate}
    \item \textbf{One-to-one.} A single shape maps to a single region
      (Figure~\ref{fig:cases}). \maneesh{Not sure I see this case in
      Figure 5. We should label the figure so the correspondence is
      clear.}
    \item \textbf{Forward many-to-one.} Multiple shapes map to a
      single region but remain distinct objects, \eg when similarly
      colored objects from frame $t - 1$ collide in frame $t$
      (Figure~\ref{fig:cases}).  \maneesh{We should stick to the terms
        ``shapes'' and ``regions'' and not use ``objects''. Not clear
        what an ``object'' is or what is means to be
        distinct. Similarly what does it mean for objects to ``merge''
        as explained in the next case.}
    \item \textbf{Backward many-to-one.} Multiple shapes map to a
      single region and merge into one object, \eg disjoint objects in
      frame $t - 1$ are part of the same object in frame $t$
      (Figure~\ref{fig:cases}).
    \item \textbf{Forward one-to-many.} A single shape maps to
      multiple regions but move consistently, \eg an object from frame
      $t - 1$ is occluded by another object in frame $t$. \maneesh{How is occlusion different from collision. I think we want to be careful about these two terms.}
    \item \textbf{Backward one-to-many.} A single shape maps to
      multiple regions and splits into new shapes, \eg a single object
      at time $t - 1$ separates into several new objects at time $t$.
\end{enumerate}

Note that valid mappings require at least one of $|S| = 1$ or $|R| =
1$. The graph $B$ can be considered a set of (potentially invalid)
undirected mappings. We will use the differentiable compositing
framework~\cite{} to extract valid directed mappings from $B$.
\maneesh{Need to explain ahead of time why many-to-many is invalid in
  terms of the graph. We need to introduce the differential
  compositing approach earlier in the overview rather than talking
  about it here for the first time. We also probably need to describe the basics of that method here, succinctly (no more than 1 short paragraph) but in enough detail that a reader can get the basics what that technique takes as input, what it reports as output a 1 sentence description of how it does it. Need to explain it is asymmetric in the sense that the optimization will be different depending on whether shapes are optimized against regions or vice versa.}

\begin{figure*}
    \centering
    \includegraphics[width=0.45\textwidth]{skeleton_figs/forward_mappings.png}
    \includegraphics[width=0.45\textwidth]{skeleton_figs/backward_mappings.png}
    \caption{Fine mappings.}
    \label{fig:fine_mapping}
\end{figure*}

For each connected component $(\mathcal{S}_k, \mathcal{R}_k)$ in $B$,
we jointly optimize the affine parameters (scale, rotation, skew and
translation) and z-index of all shapes in $\mathcal{S}_k$ to match the
target appearance of the regions $\mathcal{R}_k$. \maneesh{The
  subscripts are confusing. Are they frame times or are they Shape and
  Region indices. Why are they the same for Shapes and Regions? Also
  we need to explain our focus on affine motion models as one of the
  assumptions earlier on. Forward/backward loss is confusing because
  we also use forward/backward flow which is different. Perhaps we
  should try to find different words for these losses.} This gives us
a \textit{forward loss}. We then repeat the same process again but
instead optimize the same variables for the regions to match the
target appearance of the shapes. This gives us a \textit{backward
  loss}. The reasoning behind using both directions is that objects
may collide to form a single region, or they may separate into multiple
regions. The forward loss will be low and the backwards loss will be
high in the first scenario, and vice versa in the second scenario.
\maneesh{I think the reasoning needs to come up front -- probably before the bullet point list of cases. Always try to explain why before explaining what is done.}

Once the optimization has converged, we proceed to collect all \textit{candidate} valid mappings. For each shape $S_i \in \mathcal{S}_{t - 1}$, we compute 
\begin{equation}\label{eq:max_in_region}
    R_i = \text{argmax}_{R_j \in \mathcal{R}_t} \, \frac{|S_i \cap R_j|}{|S_i|} 
\end{equation}
as well as
\begin{equation}\label{eq:max_over_region}
    \mathcal{R}_i = \bigg\{ \, R_j \in \mathcal{R}_t \, \text{ s.t } \, \frac{|S_i \cap R_j|}{|R_j|} > \alpha \, \bigg\} \subseteq \mathcal{R}_t.
\end{equation}
\maneesh{unclear what the subscripts are indexing over.}  Note that we
overload $S_i$ and use it to denote $S_i$ warped by the affine
transformation computed in the optimization. \maneesh{I wouldn't overload the notation. Better to introduce a new variable.} Colloquially, the region
in Equation~(\ref{eq:max_in_region}) is the region which $S_i$
overlaps with the most, and the regions in
Equation~(\ref{eq:max_over_region}) are all regions who are covered by
$S_i$ in more than a fraction of $\alpha$ (we use $\alpha = 0.9$). \maneesh{Would use a different variable than alpha for this threshold as that can be confused with the notion of alpha for compositing.}

Each set $\mathcal{R}_i$ determines a valid mapping $S_i \rightarrow
\mathcal{R}_i$, so we add that to our set of candidate mappings. To
find the valid mappings in the opposite direction, we define a
bipartite directed graph $B' = (\mathcal{S}_{t - 1},
\mathcal{R}_t)$. The region found in Equation~(\ref{eq:max_in_region})
is kept track of by adding an edge $S_i \rightarrow R_i$ to
$B'$. After iterating through all $S_i \in \mathcal{S}_{t - 1}$, we
add all connected components of $B'$ (which have the form
$\mathcal{S}_{t - 1} \supseteq \mathcal{S}_j \rightarrow R_j $) to our
set of candidate mappings. \maneesh{Unclear to me why we need $B'$ and why we can't just use the inverse process to compute valid backward mappings. I think I am a little confused by the description at this point.}

Every mapping is also assigned a score equal to the masked $L_2$ RGB
loss between the optimized shapes and mapped regions. Thus, a lower
score indicates a better mapping. This entire process is then repeated
in the $\leftarrow$ direction, \ie switching the roles of
$\mathcal{S}_{t - 1}$ and $\mathcal{R}_t$. This gives us our complete
set of candidate mappings.

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{skeleton_figs/mapping_selection.png}
    \caption{Valid mapping selection.}
    \label{fig:mapping_selection}
\end{figure}

Once we have our candidate mappings, we iterate through the set and
select valid mappings to keep in a greedy fashion. When a mapping is
selected, we also remove any conflicting mappings from the set. A
conflicting mapping is another mapping which contains any overlap in
shapes or regions with the selected mapping. We also only add mappings
if their score is lower than some user-set threshold. The full process
is described in Algorithm~\ref{alg:mappings}.

\begin{algorithm}
\caption{Selecting valid mappings}\label{alg:mappings}
$\text{Given a set of candidate mappings } \mathcal{M}, \alpha$;

$\mathcal{M}^* \gets {}$;

\While{$|\mathcal{M}| > 0$}
{
    $M^* \gets \text{argmin}_{M \in \mathcal{M}} \texttt{score}(M)$;

    \For{$M \in \mathcal{M}$}{
        \If{$|\texttt{shapes}(M) \cap \texttt{shapes}(M^*)| > 0$ \text{ or } \\
        $|\texttt{regions}(M) \cap \texttt{regions}(M^*)| > 0$}{
            $\mathcal{M}. \texttt{remove}(M)$;
        }
    }

    \If{$\texttt{score}(M^*) > \alpha$}{
        $\mathcal{M}^*. \texttt{add}(M^*)$;
    }

    \Return{$\mathcal{M}^*$};
}
\end{algorithm}

% The result of the first stage is a weighted undirected bipartite graph $B$. In this next stage, we transform this graph into a weighted \textit{directed} bipartite graph $B'$ via the differentiable compositing optimization framework~\cite{}.

% For each connected component $(\mathcal{S}_k, \mathcal{R}_k)$ in $B$, we jointly optimize the affine parameters (scale, rotation, skew and translation) and z-index of all shapes in $\mathcal{S}_k$ to match the target appearance of the regions $\mathcal{R}_k$. This gives us a \textit{forward loss}. We then repeat the same process again but instead optimize the same variables for the regions to match the target appearance of the shapes. This gives us a \textit{backward loss}. The reasoning behind using both directions is that objects may collide into a single region, or they may separate into multiple regions. The forward loss will be low and the backwards loss will be high in the first scenario, and vice versa in the second scenario.

% Once the optimization has converged, we proceed to add edges into $B'$. For each shape $S_i \in \mathcal{S}_k$, we compute 
% \begin{equation}\label{eq:max_in_region}
%     R_i = \text{argmax}_{R_j \in \mathcal{R}_k} \, |S_i \cap R_j| / |S_i| 
% \end{equation}
% as well as
% \begin{equation}\label{eq:max_over_region}
%     \{R_j \, \text{s.t.} \, |S_i \cap R_j| / |R_j| > \alpha, \, R_j \in \mathcal{R}_i \},
% \end{equation}
% where we overload $S_i$ and use it to denote $S_i$ warped by the affine transformation computed in the optimization. Colloquially, the region in Equation~(\ref{eq:max_in_region}) is the region which $S_i$ relatively overlaps with the most, and the regions in Equation~(\ref{eq:max_over_region}) are all regions who are covered by $S_i$ in more than a fraction of $\alpha$. We add edges $(S_i \rightarrow R_i)$ and $(S_i \rightarrow R_j)$ for each $j$ computed in Equation~(\ref{eq:max_over_region}). The weight of each edge is the masked L2 loss in RGB space between $S_i$ and all the aforementioned regions. We also add the score from the corresponding unweighted edge in $B$, though we take the inverse exponential $e^{-x}$ of that score (since lower is better in the RGB loss). We repeat this same process in the backwards direction, which gives us weighted edges from regions to shapes (though not necessarily connecting the same shapes and regions).

\subsubsection{Region identification}\label{identification}

% Propagating identifiers from shapes to regions can occur in multiple ways, as shown in Fig.~\ref{fig:cases}. These cases roughly correspond to how objects overlap, split, merge and collide. In total, we identify five different possible scenarios:

% \begin{enumerate}
%     \item \textbf{One-to-one.} A single shape maps to a single region (Figure~\ref{fig:cases}).
%     \item \textbf{Forward many-to-one.} Multiple shapes map to a single region but remain distinct objects, \eg when similarly colored objects from frame $t - 1$ collide in frame $t$ (Figure~\ref{fig:cases}).
%     \item \textbf{Backward many-to-one.} Multiple shapes map to a single region and merge into one object, \eg disjoint objects in frame $t - 1$ are revealed to be part of the same object in frame $t$ (Figure~\ref{fig:cases}).
%     \item \textbf{Forward one-to-many.} A single shape maps to multiple regions but move consistently, \eg an object from frame $t - 1$ is occluded by another object in frame $t$.
%     \item \textbf{Backward one-to-many.} A single shape maps to multiple regions and splits into new shapes, \eg a single object at time $t - 1$ separates into several new objects at time $t$.
% \end{enumerate}

% We require our graph $B'$ to only contain connected components which fall into one of the five categories described above. To ensure this, we repeatedly remove edges from $B'$ until this property is true. We proceed to remove edges in a greedy fashion, seeking to preserve all high priority mappings and removing edges which conflict with them. Given the graph $B' = (\mathcal{S}_{t - 1}, \mathcal{R}_t)$, we follow Algorithm~\ref{alg:mappings} to generate our final mappings.

% \begin{algorithm}
% \caption{Shape-region bipartite mapping}\label{alg:mappings}
% $\text{Given } B' = (\mathcal{S}_{t - 1}, \mathcal{R}_t), \, \texttt{stable} \gets False, \, \texttt{visited} \gets \{\}$;

% \While{not \texttt{stable}}
% {
%     $\texttt{stable} \gets True$;
    
%     $v^* \gets \text{argmin}_{v \in V(B') \, \backslash \, \texttt{visited}} \; \min (\texttt{avg\_in}(v), \texttt{avg\_out}(v))$;

%     $\texttt{visited}[v^*] \gets True$;

%     \uIf{$\texttt{avg\_in}(v^*) < \texttt{avg\_out}(v)$}{
%         $\texttt{stable} \gets False$;
    
%         $\text{remove all } e \in E_{\text{out}}(v^*)$;
        
%         \For{$u \in \texttt{adj\_in}(v^*)$}{
%             $\text{remove all } e \in E_{\text{out}}(u) \, \backslash \, \{u \rightarrow v^*\}$;
            
%             $\text{remove all } e \in E_{\text{in}}(u)$;

%             $\texttt{visited}[u] \gets True$;
%         }
%     }\Else{
%         $\texttt{stable} \gets False$;
        
%         $\text{remove all } e \in E_{\text{in}}(v^*)$;

%         $\texttt{visited}[v^*] \gets True$;
        
%         \For{$u \in \texttt{adj\_out}(v^*)$}{
%             $\text{remove all } e \in E_{\text{in}}(u) \, \backslash \, \{u \rightarrow v^*\}$;

%             $\text{remove all } e \in E_{\text{out}}(u)$;

%             $\texttt{visited}[u] \gets True$;
%         }
%     }
% }
% \end{algorithm}

% We want a directed mapping graph that is bipartite with no paths from A back to A unless it is representing a 1:1 match.

Given our set of valid mappings $\mathcal{M}^*$, we propagate the identifiers from frame $t - 1$ to frame $t$ as follows:
% Note: Each pixel can have multiple labels

\begin{itemize}
    \item \textbf{One-to-one.} We label the region with the identifier of the matched shape.
    \item \textbf{Forward many-to-one.} For each shape $S_i$ mapped to the region, we label the area of the region which was covered by $S_i$ after the optimization with the identifier of $S_i$. Note that a single pixel in frame $t$ can have multiple identifiers assigned to it. \maneesh{Not sure I understand why we are labeling things this way. Probably I just don't know what the case really is.}
    \item \textbf{Backward many-to-one}. We choose a single canonical identifier from one of the mapped shapes and assign that identifier to the region. We also relabel all shapes previously identified with any of the mapped shapes' identifiers with the canonical identifier.
    
    \sharon{NOTE: Merging has not been completely determined yet. Right now, I merge all previous appearances of any identifier within the ``equivalence class" and re-identify them with the canonical identifier, but this may result in disjoint objects being merged into one identifier. I could also only relabel the identifiers at time $t - 1$.}
    
    \item \textbf{Forward one-to-many.} We label all regions with the identifier of the matched shape.
    \item \textbf{Backward one-to-many.} We give unique new identifiers to each of the regions.
\end{itemize}

Finally, any remaining unidentified regions or pixels are given new unique identifiers, and the mask of every identified object is saved.

\subsubsection{Canonical object appearances}

In order to meaningfully determine affine transformations of an object
at each frame, we need to maintain a canonical object appearance.
\maneesh{I'm not sure what is ``meaningful'' about the canonical object appearance. It might be better to just say that we consider the highest resolution, occlusion-free version of the object as the canonical appearance -- thought we should need to explain how we check for occlusions.}
We
keep track of this by saving the ``best" appearance of each object as
it is tracked. We begin with the initial appearance of an object when
it is a new region that is first identified, and then update the
appearance whenever it is identified unoccluded and covering more
pixels in a later frame.

\subsection{Affine transform optimization}
After the object tracking stage we obtain a set of objects, each
associated with an appearance and object mask at every frame in which
it appears. The final step is to determine the affine transformations
between the canonical appearance of each object and its appearance at
each of those frames. For each object in a single frame, we have the
canonical object appearance and the target object appearance
(determined by the object masks saved from the previous phase). We use
the differentiable compositing optimization framework to determine
this transformation. The transformation parameters (scale, rotation,
skew and translation) along with the z-index are written out to the
final program.
\maneesh{We probably need to explain why another optimization is necessary here. It seems like it shouldn't really need to be optimized again. Perhaps to get a little bit better fit.
  But I contend that it should be possible to get the transformations from the sequence of transformations that was computed frame to frame. }

\subsubsection{Optimization initialization}
Given an arbitrary shape, the optimization process may converge to
many local minima that represent affine transformations far from the
correct transform.  \sharon{Add a visual example of local minima
  resulting from poor rotation/translation initializations.}
\maneesh{I don't think we need to explain why the optimization needs good initialization. The readers
  will know this. We can simply explain that we can obtain a good initialization as follows. But do we need to do that via the optical flow.
I think it would be better to initialize using the transformations we've computed in the optimizations performed earlier in the matching process.}
To avoid
recording an incorrect transform, we initialize the rotation and scale
of each object at time $t$ using the optical flow
$\overrightarrow{F}_{t - 1}$. At the first frame, we do not have an
optical flow computation, so we search over all rotations
$[-180^\circ, 180^\circ)$ in increments of one degree. For each
  rotation angle, we apply the rotation to the object and then scale
  it to fit within the bounding box of the object mask at that
  frame. We select the rotation angle $\theta$ which minimizes the RGB
  loss. The initial scale parameters are then determined by rotating
  the rotated and scaled object by $-\theta$, and then rescaling it to
  fit the size of the canonical object appearance. In total, the
  transforms applied to the canonical appearance $S_i$ are
\begin{equation}
    S^{-1}_\text{init} R^{-1}_\text{init} S_\text{box} R_\text{init} S_i,
\end{equation}
where $R_\text{init}$ is the initialized rotation by $\theta$,
$S_\text{box}$ is the scale transform to fit it into the bounding box
of the target mask, and $S_\text{init}$ are the initialized scale
parameters. This ``fallback" initialization is also used if the
converged optimization error for a particular object was too high in
the previous frame. \maneesh{I think we can make this paragraph more succinct as most of it is explaining the case where we don't have optical flow and that maybe can be more simply stated as being done via template matching over rotation and scale at one degree increments, or some such.}

% LocalWords:  TODO colorspace luminance Zhang centroid rgb Sintel
% LocalWords:  pretrained Hellinger efd amongst parens subsubsections
% LocalWords:  Hel undirected argmax argmin unoccluded rescaling init
% LocalWords:  initializations


==> pipeline_i.tex <==
\subsection{Region extraction}\label{sec:pipeline_i}

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{skeleton_figs/region_extraction.png}
    \caption{Region extraction. \sharon{Do you think the figure is necessary here? I am thinking of removing it.} \maneesh{Agree. we don't need a figure.}}
    \label{fig:region_extraction}
\end{figure}

Our region extraction method is an edge-based segmentation
approach. Given a frame $F$ of the input motion graphics video, we first convert it to LAB colorspace and perform a color-based foreground-background segmentation. We treat the mode LAB color as the background color, and mark any pixels which are less than some threshold distance from the background color as background pixels.
Next, we apply a Canny edge detector~\cite{} on the luminance channel to
generate a binary edge image. We drop all edge pixels which fall on the background region. Using the edges as boundaries, we compute foreground regions $\mathcal{R} = \{ R_1, \ldots, R_N \}$ using the trapped-ball
segmentation method of Zhang~\etal~\cite{}.
\maneesh{I might use lowercase $f$ for frames. Let's talk about this.}
\maneesh{I wonder if instead of a solid background we could assume a static background and use a separation method that deals with textured/gradient backgrounds. Let's see if we have time for this.}
% \maneesh{ Last sentence is  also confusing because it is unclear what an ``object'' is. I modified the sentence a bit to clarify, but we do need to explain somewhere what a foreground object is -- perhaps at beginning of next subsection.}

% LocalWords:  colorspace luminance Zhang


==> pipeline_ii.tex <==
\subsection{Object identification}\label{sec:pipeline_ii}
\begin{figure*}
    \centering
    \includegraphics{figs/cases-01.png}
    \caption{Label propagation cases.}
    \label{fig:cases}
\end{figure*}

\maneesh{Move to lowercase r and o for individual regions and objects and uppercase or mathcal uppercase for sets of such things?}
\sharon{Since regions/objects can be considered lots of pixels I wanted to separate them from constants/numbers that are more like ``one" entity, but I think mathcal uppercase would make sense for all sets.}

Given a set of regions for every input frame, our goal is to identify
unique objects and track them from frame to frame.  We initialize this
process at the first frame $F_1$, by treating each
region $R_i \in \mathcal{R}_1$ as an object $O_i$ so that
\begin{equation}
  \mathcal{O}_1 = \{O_i = R_i | \forall R_i \in  \mathcal{R}_1\},
\end{equation}
and assigning each such object $O_i$ a unique ID.
%
%For each subsequent frame $F_t$, our task is to assign object IDs to
%the pixels of each region $R_i$ in $\mathcal{R}_t$, thereby converting each
%such region into one or more objects. \maneesh{Do we need the final phrase, starting at ``thereby''}
%
%Our approach is to reuse object IDs from the previous frame whereever
%we can construct affine transformations that map objects in the
%previous frame $\mathcal{O}_{t_1}$ to region pixels in the current
%frame $\mathcal{R}_{t_1}$, or vice versa. Such reuse occurs when an
%existing object moves from frame to frame.  If no such affine
%transformation(s) exist we assign the region pixels a new unique
%object ID and treat the collection of such pixels as a new object.
%
%Specifically, we must determine when objects $\mathcal{O}_{t-1}$ and
%their corresponding IDs from the previous frame can be
%assigned to region pixels in the current frame (indicating affine motions of
%existing objects) and when we must introduce a new unique object ID for
%the region pixels (indicating the appearance of a new object).
%
%Specifically we must determine how objects from the previous frame $\mathcal{O}_{t-1}$
%map to regions in the current frame $\mathcal{R}_{t}$ under affine transformations.
%
For each subsequent frame $F_t$, our task is to determine how objects from the previous frame
map to regions in the current frame $\mathcal{R}_{t}$ under affine transformations.
%
%Figure~\ref{fig;cases} shows \maneesh{XX} cases that can occur when
%assigning objects $\mathcal{O}_{t_i}} and their corresponding IDs in
%  the previous frame to the region pixels in the current frame.
%Figure~\ref{fig:cases} shows the \maneesh{XX} cases that can occur when determining these mappings:
Figure~\ref{fig:cases} shows the \maneesh{XX} types of mappings that can occur between objects and regions.
\begin{enumerate}
\item \textbf{One-to-one.} A single object maps to all pixels in a
  single region under a single affine transform.  %Object 1 in
  %Figure~\ref{fig:cases} is an example of this case.

  \item \textbf{Unmatched object or region.} A single object or region does not map to any region or object. We consider this to be the case where an object disappears from or first appears in the video. \sharon{I should mention this in assumptions? Since we do not track objects anymore once they have disappeared.} \maneesh{Need to split into appear and disappear cases.}
  
\item \textbf{Many-to-one (merge).} Two or more objects 
  map to a single region under a single affine transform, mapping the region to all the objects.
  Because a single affine motion explains
  how the region moves to match all the objects, we consider this a merging of the distinct
  objects.
  %We assign a new object ID to the region and propagate the
  %  new ID back to all previous objects involved in the merge.
  %  Objects 3
  %  and 4 merge to form object XX in Figure~\ref{fig:cases}, as the dark blue H is entering the scene.
  
\item \textbf{Many-to-one (no merge).} Two or more objects map to a
  single region, but a different affine transformation is required to warp
  each object to the region. Since multiple transformations are needed to explain how the
  objects move to match the region, we do not treat this case as a merge but
  instead consider the objects to remain distinct while touching or overlapping as they map to a single region.
%  rather as two or more objects moving so that they overlap
%  or touch one another in the current frame. The objects remain distinct even though they map to a single region.
  %
%  \maneesh{Rest of item might get cut or shortened.}
%  Since multiple transformations are required to explain how the
%  objects move to match the region pixels we do not merge the objects. Instead we transform each
%  object and assign the overlapped region pixels the corresponding
%  object ID. Note that when region pixels overlap more than one object
%  we maintain all overlapping object IDs for those region pixels.  In
%  Figure~\ref{fig:cases} objects 7 and 8 continue to exist as pieces of
%  the corresponding region in frame $t$.
  
\item \textbf{One-to-many (split).} A single object maps two or more
  regions but a different affine transformation is required for each
  one. This is the inverse of the many-to-one (no merge) case,
  but here we consider the object as splitting into multiple pieces.
  %
%  \maneesh{Rest of item might get shortened.}
%  But here,
%  a single object is splitting into multiple regions, and therefore we
%  assign each such region a new unique object IDs.  In
%  Figure~\ref{fig:cases} two different regions map to object 2 with differing
%  transformations and so we split object 2 into new objects XX and YY.

\item \textbf{One-to-many (no split).} A single object maps to two or
  more regions under a single affine transform.  This is the inverse
  of the many-to-one (merge) case, 
  but here we consider the object as being occluded by another object or the edge of the frame rather
  than splitting into pieces.
  %
%  \maneesh{Rest of item might get shortened.}
%  But here, since we have a single
%  object, we assign its ID to all of the regions. In
%  Figure~\ref{fig:cases}, the ID of object 9 is assigned to both
%  regions in frame $t$.

\item \textbf{Many-to-many (split and merge).} Multiple objects map to
  multiple regions under differing affine transforms. In this case
  objects are splitting apart and simultaneously merging with other objects.
%  In Figure~\ref{fig:cases} objects 5 merges with part of object 6,
%  while object 6 splits out the circle.
  Because both splits and merges are
  involved it is ambiguous how the objects map to the regions. We discuss how
  we handle this case in Section~\ref{sec:}.
  \maneesh{May need to say this case is uncommon.}
   \maneesh{Not sure the example in Fig 4 is
    correct. Both elements in frame t-1 and t must consist of two
    objects. So we need 4 objects all together and there needs to be a
    flip in which ones are connected as a single region.}
    \sharon{I think the figure does map both objects to both objects? The arrow are wrong though, there shouldn't be an arrow from the top left to the lower right.}
\end{enumerate}

\maneesh{We need to add cases of objects appearing and disappearing?}

\maneesh{I removed explanation of what we do to propagate IDs from cases. That is implementation detail and here we should be focusing on what can happen in a video in terms of mappings. We should explain how we propagate IDs later.}


To determine which of these mapping types best match previous frame
objects $\mathcal{O}_{t-1}$ with current frame regions $\mathcal{R}_t$
we take a \maneesh{XX} step approach.
%
In the first step we construct a bipartite
graph $B = (\mathcal{O}_{t - 1}, \mathcal{R}_t)$ where each edge
indicates a likely correspondence between an object and region (Section~\ref{}).
%
In the second step we use the graph to extract a set of likely mapping type hypotheses
between the objects and regions (Section~\ref{}).
%
In the third step we score each mapping type hypothesis (Section~\ref{}).
%
And in the fourth step we select the set of mappings that collectively
best explain how objects move from the previous frame to the current
frame, using a greedy approach (Section~\ref{}).
%
\maneesh{May need to add something on label ID propagation.}


\subsubsection{Step 1: Build bipartite correspondence graph}
\label{sec:bipartite}

To build the bipartite correspondence graph $B$ between objects
$\mathcal{O}_{t - 1}$ and regions $\mathcal{R}_t$ we start with a
complete graph containing an edge $(O_i, R_j)$ between every object
$O_i \in \mathcal{O}_{t-1}$ and every region $R_j \in \mathcal{R}_t$.
We then compute a weight for each edge, that describes how strong the
correspondence is between the object and the region.
This
correspondence weight is determined by a combination of shape, color
and optical flow features as
\begin{equation}
  W(O_i,R_j) = W_{shp}(O_i,R_j)\cdot W_{clr}(O_i,R_j) \cdot W_{flow}(O_i,R_j).
\end{equation}

For the shape correspondence weight $W_{shp}(O_i,R_j)$ we represent
the contours of both the object and the region using
the first 36 terms of their elliptic Fourier descriptors~\cite{} and then
take the cosine similarity between them as
\begin{equation}
  W_{shp}(O_i,R_j) = | \langle \text{F}(O_i), \text{F}(R_j) \rangle |.
\end{equation}
\maneesh{Can we use a single letter -- F maybe to represent EFD?}
Using the elliptic Fourier descriptors in this manner makes this weight more robust to small deformations of the contours.
\maneesh{Not sure the prev sentence is quite right.}
\sharon{The EFD works better in distinguishing shapes as contours have higher frequencies. I don't think in our videos we leverage this very much, and actually in many cases the shapes are quite simple, but it is able to distinguish a good amount of different objects.}

For the color correspondence weight $W_{shp}(O_i,R_j)$ we build
a 64 bin color histogram in LAB space for the object $H_\text{LAB}(O_i)$ and the region $H_\text{LAB}(R_j)$ and then
compute the Hellinger distance between these histograms as
\begin{equation}
  W_{clr}(O_i,R_j) = 1.0 - d_\text{Hel}(H_\text{LAB}(O_i), H_\text{LAB}(R_j)).
\end{equation}
\sharon{The Hellinger distance measures the similarity between distributions and is bounded in $[0, 1]$, making it comparable in scale to our other scores.}
\maneesh{Explain why we use Hellinger distance.Also is this one a distance or a similarity. I think we want the latter.}
\sharon{I think it is a metric, but the inversion described in the equation is a similarity score.}


For the flow correspondence weight $W_{flow}(O_i,R_j)$ we use
RAFT~\cite{}, a deep neural network architecture for computing optical
flow that was pretrained on the Sintel~\cite{} dataset. \sharon{This dataset contains videos from a 3D animated short film. We chose this model because the data consists of computer-generated imagery rather than natural images.} \maneesh{Does
  this dataset match the characteristics of our data? If so we should
  say that.} \sharon{I just looked into other optical flow datasets. It may be possible to train our own version of RAFT using those other cartoon animation datasets.} Specifically, we use RAFT to compute the forward optical
flow ($\overrightarrow{\mathcal{F}}(O_i,R_j)$) from the previous frame
object to the current frame region, and we similarly similarly the
backward optical flow ($\overleftarrow{\mathcal{F}}(O_i,R_j)$). These
flow functions compute dense optical flow vectors and then advect the
pixels along the flow vectors. We then compute the flow correspondence weight as
\begin{equation}
  W_{flow}(O_i,R_j) = \frac{ |\overrightarrow{\mathcal{F}}(O_i,R_j) \cap R_j| + |O_i \cap \overleftarrow{\mathcal{F}}(O_i,R_j)| } {2}.
\end{equation}
The forward intersection term $|\overrightarrow{\mathcal{F}}(O_i,R_j) \cap R_j|$ checks how well
the forward motion of the object matches the pixels of the region while the backward intersection
term $|O_i \cap \overleftarrow{\mathcal{F}}(O_i,R_j)|$ checks the match when moving the backwards.
\maneesh{Do we advect or does RAFT compute a transform (affine?) using RANSAC on the optical flow?} \sharon{We advect, the RANSAC has to be done separately with the pixel-wise flow information and RAFT does not compute that for us.}

Once we have computed the correspondence weight for each edge in the
complete bipartite graph, we drop any edge with a weight of zero, leaving
us with a set of likely correspondences between objects and regions.

\subsubsection{Step 2: Extract mapping type hypotheses}
\label{sec:extractMappingHypotheses}
The bipartite graph $B$ resulting from step 1 contains likely
correspondences between objects and regions. In this step we use $B$
to extract a set of hypotheses for the possible mapping types between
the objects and regions.

%The bipartite correspondence graph $B$ resulting from step 1 contains
%a set of hypotheses for the possible mapping types between objects and
%regions.  In this step we extract each such mapping type hypothesis and then
%compute its likelihood score.
%
%Both the extraction and scoring computations are based on an extension
Our extraction process uses an extension
of Reddy et al.'s~\cite{} differentiable image compositing
optimization technique that we have adapted to our problem setting. We
first describe this optimization, then how we extract the mapping
hypotheses.% and finally how we score each extracted mapping.

\paragraph{Differentiable image compositing}
Graphic patterns are static images composed of discrete elements
(e.g. shapes with solid colors, simple gradients or basic textures)
that may partially occlude one another.  Differentiable image
compositing~\cite{} is an optimization technique that can de-composite
such patterns into a layered representation.  As input it takes a {\em
  target} pattern image $T$ along with a set of {\em source} element
template images $\mathcal{S} = \{S_1...S_N\}$ that appear in the
pattern.  It jointly optimizes the parameters of a similarity transform (i.e.,
translation, rotation and uniform scale) for each source element and
their visibility ordering so that when the elements are rendered in
back-to-front order they reproduce the target pattern.  Thus we write
the discrete compositing (DC) optimization function as
\begin{equation}
\text{DC}(\mathcal{S} = \{S_1...S_N\}, T) = \{(S_i, \Theta_i, \Lambda_i) | \forall S_i \in \mathcal{S} \},
\end{equation}
where $\Theta_i$ is the transform that maps element $S_i$ to it's
placement in $T$, and $\Lambda_i$ is an integer z-order layer number
(larger z's are in front of lower z's) for element $S_i$ with
respect to the other elements in $\mathcal{S}$ after they have been
transformed by their respective $\Theta$'s.

With this information we can, for example, generate the composite
image $\mathcal{I}^\text{cmp}(\Theta(\mathcal{S}))$ of the set of
source elements $\mathcal{S}$ after they have all been placed in $T$
according to their $\Theta$'s and composited using their $\Lambda$'s.
Similarly we can build a binary mask
$M^\text{vis}_i(\Theta_i(S_i))$ of the visible parts of $S_i$ with
respect to the other elements in $\mathcal{S}$ after they have all
been placed and composited.
%With this information we can, for example, compute a binary mask
%$M^\text{vis}_i(\Theta_i(S_i))$ of the visible parts of $S_i$ with
%respect to the other elements in $\mathcal{S}$ after they have all
%been placed in $T$ according to their $\Theta$'s and composited using their
%$\Lambda$'s.
\maneesh{Technically $M^\text{vis}$ needs access to all the
  information produced by DC. I've dropped this to hopefully improve
  clarity. We may need figures to help show this.}

Frames of motion graphics video often appear visually similar to
graphic patterns with foreground objects possibly occluding one
another layered on a background. However we have found that affine
motion transforms (i.e., translation, rotation, non-uniform scale and
shear) are more common in motion graphics than similarity transforms.
Thus we extend the DC optimization technique to explicitly compute an
affine transformation $\Theta(S_i)$ that maps each source element
$S_i$ to its placement in the target image.  Specifically we add
transformation parameters for x-scale, y-scale, x-shear and y-shear as
independent variables in the optimization.  \maneesh{Should we say
  something about removing overlap loss -- they used to account for
  overpopulating with template elements.}

\sharon{I would call this a scoring function instead of a loss function.}
We also  use the information provided by the DC optimization to define
a new loss function $\mathcal{L}_\text{vis}$ that compares how well a
source element $S_i$ matches the target image $T$ while properly
accounting for visibility as,
%after being transformed by $\Theta_i$ while
%accounting for occlusions given by $\Lambda_i$, as
\begin{equation}
  \mathcal{L}_\text{vis}(S_i,T) = \mathcal{L}_\text{int}(S_i,T) + \mathcal{L}_\text{xor}(S_i,T).
\end{equation}
The first term $\mathcal{L}_\text{int}$ measures the $l^2-norm$ color difference between the
visible pixels of $S_i$ and corresponding pixels in $T$ wherever they intersect in the target space. Specifically,
\begin{equation}
  \mathcal{L}_\text{int} = ||M^\text{int} \otimes (\Theta_i(S_i) - T)||_2,
\end{equation}
where $\otimes$ denotes the pixel-wise multiplication operator, and
$M_\text{int}$ is a binary mask representing the pixels of $Theta_i(S_i)$ that
are visible in the target space, $M^\text{vis}_i(\Theta_i(S_i))$ and that are
also within $T$. That is,
\begin{equation}
  M^\text{int} = M^\text{vis}_i(\Theta_i(S_i)) \cap T.
\end{equation}
The second term $\mathcal{L}_\text{xor}$ penalizes the areas where
$\Theta_i(S_i)$ and $T$ do not align -- i.e., pixels {\em only} occupied by
$\Theta_i(S_i)$ or {\em only} by $T$, as
\begin{equation}
  \mathcal{L}_\text{xor} = \frac{|M^\text{vis}_i(\Theta_i(S_i)) \oplus T|}{|M^\text{vis}_i(\Theta_i(S_i)) \cup T |}. 
\end{equation}
Here, $\oplus$ denotes the pixel-wise XOR operator and the ratio
computes the mismatched area between $\Theta_i(S_i)$ and $T$ as a
percentage of the total area covered by them.

\maneesh{May not need to discuss the stuff in this finally paragraph or discuss DC on target set earlier before Loss and talk about loss in terms of sets..}
Finally we extend the DC optimization function to take a set of target elements $\mathcal{T}$
rather than a single target image $T$ as input and internally composite all of them into
a single target image before applying the optimization. That is
\begin{equation}
  %  \text{DC}(\mathcal{S} = \{S_1...S_N\}, \mathcal{T} = \{T_1...T_M\}) = DC(\mathcal{S}, \bigcup_{j=1}^MT_j).
    \text{DC}(\mathcal{S} = \{S_1...S_N\}, \mathcal{T} = \{T_1...T_M\}) = DC(\mathcal{S}, \mathcal{I}^\text{cmp}(\mathcal{T})).
\end{equation}
\sharon{Maybe we can skip the previous info--our target is not really composited either, it is just pulled from the frame. So it is pretty similar to the target image used in the original DC paper.}
Note that because the target elements do not have a layering
associated with them we composite them in an arbitrary order.
Internally we keep track of where the individual target elements lie
within the union so that in this setting we can also compute the
visibility loss of a source element $S_i$ against a specific target
element $T_j$ as $\mathcal{L}_\text{vis}(S_i,T_j)$.
%
We similarly extend $\mathcal{L}_\text{vis}$ to take a
set of source images as input as,
\begin{eqnarray}
  \mathcal{L}_\text{vis}(\mathcal{S},T) &=& \mathcal{L}_\text{int}(\mathcal{S},T) + \mathcal{L}_\text{xor}(\mathcal{S},T),\\
  \mathcal{L}_\text{int} &=& ||M^\text{int} \otimes (\mathcal{I}^\text{cmp}(\Theta(S)) - T)||_2,\\
  M^\text{int} &=&  \bigcup_{i=1}^N M^\text{vis}_i(\Theta_i(S_i)) \cap T,\\
    \mathcal{L}_\text{xor} &=& \frac{|\bigcup_{i=1}^N M^\text{vis}_i(\Theta_i(S_i)) \oplus T|}{|\bigcup_{i=1}^N M^\text{vis}_i(\Theta_i(S_i)) \cup T |}. 
\end{eqnarray}
\maneesh{Seems like way too much detail and space. How can we shorten.}
\sharon{Define once for multiple objects?}



\maneesh{I think this paragraph on initialization is too much detail and should be removed.}
In this paper we apply the adapted DC optimization to match source
object(s)s to a composite image containing one or more regions, or
vice versa (i.e., we align source region(s) to composite target
object(s)). In either case we have found the optimization is sensitive
to initialization.  Therefore, if our RAFT~\cite{} based optical flow
weight $W_{shp}(S_i,T)$ and appearance $W_{clr}(S_i,T)$ suggest a
strong match we initialize $\Theta(S_i)$ with an affine transform
generated by applying RANSAC to the optical flow vectors of
$S_i$. Otherwise we initialize $\Theta(S_i)$ to so that $S_i$ is
translated to the centroid of $T$ and we use template matching to
compute an initial rotation and scale.



\paragraph{Extract hypotheses}
To extract the mapping type hypotheses from the correspondence graph $B$,
we build two additional graphs for each connected component $C$ of $B$;
(1) A {\em forward mapping type hypothesis graph} and (2) a {\em backward mapping type hypothesis graph}.
\maneesh{will need a figure, perhaps an algorithm }
%
To build the forward graph we first apply the differentiable
compositing optimization as,
\begin{equation}
  DC(\mathcal{O}_{t-1}^C, \mathcal{R}_t^C),
\end{equation}
treating the set of previous frame objects in the connected component
$\mathcal{O}_{t-1}^C = \{O_i | O_i \in C\}$ as the sources and the set of current frame
regions in the connected component $\mathcal{R}_t^C = \{R_j | R_j \in C\}$ as the targets.
%
\sharon{Following two equations should be intersection rather than union?}
Then for each object $O_i \in C$ we consider each edge $(O_i,R_j) \in
C$ and compute a {\em source} coverage weight as
\begin{equation}
  W_\text{cov}^\text{src}(O_i, R_j) = \frac{| \Theta_i(O_i) \cup R_j |}{|\Theta_i(O_i)|},
\end{equation}
and add the highest non-zero weighted edge to the forward graph.
%This usually adds one
%edge for each object $O_i \in C$ to the forward graph.
%
Similarly, for each region $R_j \in C$ we consider each edge
$(O_i,R_j) \in C$ and compute a {\em target} coverage weight as
\begin{equation}
  W_\text{cov}^\text{tgt}(O_i, R_j) = \frac{| \Theta_i(O_i) \cup R_j |}{|R_j|},
\end{equation}
and add the highest non-zero weighted edge to the forward graph if it has not
already been added to the graph.
%This usually adds one
%edge for each object $R_j \in C$ to the forward graph.
%
The backward graph is built in exactly the same way except that it
treats the regions $\mathcal{R}_t^C$ as sources and the objects
$\mathcal{O}_{t-1}^C$.
\maneesh{Have to note that we save the DC information with the mappings -- especially the Theta but also need the Lambda's}


Figure~\ref{fig:hypotheses} shows how both the forward and backward
graphs both encode possible mapping types. \maneesh{This Figure is
  very important and will also need to work in conjunction with Fig
  4. Mappings (both in Fig 4 and here) should always visualize the
  transformation being applied to either object(s) (fwd case) or
  region(s) (backwards case)}
%
For example, if we consider a single object $O_i$ in the forward graph
and it has a single edge $(O_i,R_j)$ then one hypothesis is that there
is a one-to-one mapping from $O_i$ to $R_j$.  If $O_i$ has multiple
edges in the forward graph then a hypothesis is a one-to-many (no
split) mapping from $O_i$ to each of the regions it is connected
to. Alternatively if a single region $R_j$ is connected to multiple
objects in the forward graph, the corresponding hypothesis is a
many-to-one (no merge) mapping. \maneesh{May want to highlight that all mapping hypotheses
in the forward graph have transforms Theta on edges that map objects to regions.}
%
The backward graph similarly encodes one-to-one, many-to-one (merge)
and one-to-many (split) mapping type hypotheses.
%
\maneesh{May want to highlight that all mapping hypotheses
in the backward graph have transforms Theta on edges that map regions to objects.}
%
\maneesh{Maybe need
  to say something about not worrying about many-to-many at this
  point.   While graphs may also provide many-to-many hypothesis, ...}


\subsubsection{Step 3: Score mapping type hypotheses}
In step 3 we compute a score for all the one-to-one, one-to-many and many-to-one
mapping hypotheses we can extract from the forward and backward
graphs. Specifically, given a mapping type hypothesis extracted from
the forward graph $\overrightarrow{\mathcal{H}}$, we set its score to
$\mathcal{L}_\text{vis}(\mathcal{O}_{t-1}^{\overrightarrow{\mathcal{H}}},\mathcal{R}^{\overrightarrow{\mathcal{H}}}_{t})$,
where $\mathcal{O}_{t-1}^{\overrightarrow{\mathcal{H}}}$ and
$\mathcal{R}^{\overrightarrow{\mathcal{H}}}$ denote sets of of
object(s) and region(s) in $\overrightarrow{\mathcal{H}}$
respectively. Similarly we score a mapping type hypothesis extracted
from the backward graph $\overleftarrow{\mathcal{H}}$ as
$\mathcal{L}_\text{vis}(\mathcal{R}_{t}^{\overleftarrow{\mathcal{H}}},\mathcal{O}^{\overleftarrow{\mathcal{H}}}_{t-1})$.


\subsubsection{Step 4: Select mapping type}
The goal of step 4 is to select a set of conflict-free mappings types
from our set of hypotheses that collectively best explain how objects
move, appear or disappear between frames $t-1$ and $t$.  A pair of
mapping type hypotheses conflict with one another, whenever they
include the same object or region (Figure~\ref{}).  \maneesh{need a
  good figure for this} Starting with our complete set of mapping type
hypotheses, our approach is to repeatedly select the mapping with the
lowest score hypotheses, then remove all conflicting hypotheses from
the set and then repeat the process. We stop once there are no more
mapping type hypotheses left in our set or the lowest score of the
remaining hypothesis a greater than a threshold $\epsilon$. We use the
threshold to reduce the chance of selecting a mapping type with a
relatively high score suggesting that the DC optimization converged to a suboptimal local minimum.
In practice we found $epsilon=??$ to provide good results across all our examples.
\maneesh{Maybe remove detail here about epsilon.}

\maneesh{Is this related to stable marriages, the liver matching algorithm or med school matching? If so maybe add a ref?}
\sharon{I don't think so, since our mappings do not consider every possible mapping encoded by the edges (e.g., we don't consider every one-to-one mapping). Thus our space of mappings is already smaller than the space that these algorithms work in.}


\sharon{------BEGIN NEW TEXT--------}

\subsection{Step 4: Propagate IDs}
Given our set of selected mappings, we can now assign IDs to the
region pixels. For \textbf{one-to-one} and \textbf{one-to-many (no
  split)} mappings, we assign all pixels of the regions with the label
of the object. For one-to-many (split) mappings and unmapped regions,
we create new IDs and label the pixels of each region with a different
ID. For many-to-one (merge) mappings, we create a new ID to assign to
the pixels of the region and then relabel all previous instances of
the object IDs in the mapping to this new ID. Finally, for many-to-one
(no merge) mappings, we assign the IDs of each object $O_i$ in the
mapping to the corresponding pixels in $\Theta_{O_i}(O_i)$.

We also keep track of a \textit{canonical appearance} for each
object. When an object first appears, we save its appearance as the
canonical appearance. Every time an object covers a larger region of
pixels in a subsequent frame, we update that canonical appearance.

\subsection{Step 5: Motion recovery}
With the frame-to-frame affine transforms and canonical appearances of
each object obtained from steps 1 through 4, we can compute affine
transforms from the canonical appearance to each frame. \sharon{This
  will require some refactoring. I've tried to write out a
  refactoring, but haven't successfully done that yet--so I'm not sure
  I can provide the math details here?} These parameters can then be
written out to the final SVG program. In practice, we found that
performing a re-optimization using the canonical appearance as the
source and the corresponding labeled pixels in each frame as the
target gives more accurate transformations.

\sharon{------END NEW TEXT--------}



\vspace{3em}
\maneesh{------OLD TEXT BELOW ------}\\

Once we have determined a set of regions for every input frame, we
proceed to identify unique objects with distinct IDs
(integer labels) and track them from frame to frame.
% \maneesh{I think
%   we need to define what a foreground object is and why it differs
%   from a region before the previous sentence.}
At each time $t$, we have a set of unidentified regions and a set of previously identified objects labeled with IDs (potentially empty).
% Any region pixel in a previous frame has been identified, and
% we call the collection of pixels identified with the same ID a
% \textit{shape} (\ie the appearance of an object in that
% frame). \sharon{is previous sentence over-complicated?} \maneesh{I
%   think the previous sentence is hard to follow -- partly because it
%   introduces a new concept of a ``shape'' without having defined
%   ``object''. We should maybe look at how previous tracking papers
%   talk about these various things -- foreground objects, shapes and
%   regions and see if we can adapt their terminology.}
We now need to determine which existing IDs should be assigned to each
pixel in the regions at the current frame, as well as what new IDs
should be created. This requires some knowledge about how the objects
in the previous frame correspond to the regions in the current frame,
which we now explain. Once we know how objects map to regions, we can
then use the corresponding object IDs to identify the regions.

\sharon{The most similar multi-object tracking language in prior work
  is modeling the problem as a bipartite graph matching problem. since
  we are not requiring one-to-one matches, I chose \textit{mapping} as
  an adjacent term. should I explain this or provide any of that
  context (maybe in the related work rather than here)?} \maneesh{We
  might talk about that in related work, or even skip it as we might
  not need to explain this relationship -- let's talk about it face to
  face and decide.}
  % We describe this task as computing an \textit{assignment mapping}.
Assume that we have tracked some objects
% \maneesh{Isn't an object in the previous frames a shape? Also I think
%   a figure will help us here showing shapes/object IDs and
%   regions. Figure should probably show the 5 cases enumerated below.}
in frames $F_1, \ldots, F_{t - 1}$. Given the next frame $F_t$ and its
regions $\mathcal{R}_t = \{ R_1, \ldots, R_N \}$, our goal is to
compute a set of \textit{mappings} between $\mathcal{R}_t$ and the objects
in $F_{t - 1}$, which we call $\mathcal{S}_{t - 1} = \{ S_1, \ldots, S_M
\}$.
% \maneesh{Before saying out goal is to compute mappings we need to explain how the mappings relate to setting the proper object IDs. I think
% we want to first introduce the various cases of what might happen (e.g. the cases listed below), then talk about how we determine which case a set of objects belongs to and then explain how we assign object IDs for each case.}
% The mapping determines how we assign identifiers to each $R_j$,
% \eg if $S_1$ is matched to $R_1$, then we assign the identifier of
% $S_1$ to $R_1$. We define five types of valid mappings:
There are six different events which may occur from time $t - 1 $ to time $t$, and each event can be represented by a different type of mapping between the objects in $\mathcal{S}_{t - 1}$ and the regions in $\mathcal{R}_t$ (see Figure~\ref{fig:cases}):
\maneesh{Let's define merges and splits in terms of have a single consistent transformation versus having multiple transformations.}
\begin{enumerate}
    \item \textbf{One-to-one.} This is the case when a single object maps to a single region, \eg object 1 in Figure~\ref{fig:cases}. In this case we should assign to $R$ the label of $S$. 
    % \maneesh{Not sure I see this case in
    %   Figure 5. We should label the figure so the correspondence is
    %   clear.}
    \item \textbf{Many-to-one (merge).} This occurs when two objects which previously received distinct IDs are now revealed to be a part of one object. For example, objects 3 and 4 in Figure~\ref{fig:cases} are revealed to be a part of one larger object that had not fully come onto frame. In this case we should merge the IDs 3 and 4 into one new ID (and relabel all previous objects accordingly).
    \item \textbf{Many-to-one (no merge).} Two objects of very similar color may come together and form one region, but not necessarily in a way that indicates they are part of one larger object. For example, object 7 and object 8 in Figure~\ref{fig:cases} both map to region G in frame $t$, but this is only due to their individual motions and not because they belong to one collective object. In this case, we want to assign both IDs 7 and 8 to the corresponding pixels in region G (including assigning \textit{both} IDs to any pixels in an area where the objects overlap).
    % \maneesh{I'm confused by this case and the ones following. Let's get a figure in place illustrating the cases and then write to the figure.}
      % \maneesh{We should stick to the terms
      %   ``shapes'' and ``regions'' and not use ``objects''. Not clear
      %   what an ``object'' is or what is means to be
      %   distinct. Similarly what does it mean for objects to ``merge''
      %   as explained in the next case.}
    \item \textbf{One-to-many (split).} When an object splits apart into multiple objects, we identify the split objects as new objects and assign new IDs to them. For instance, object 2 in Figure~\ref{fig:cases} splits apart into region C and region D, so each of those regions will receive a new, distinct object ID.
    \item \textbf{One-to-many (no split).} The inverse of case 2 (merge) may also occur, \eg when an object is exiting the frame and we only see disjoint parts of it (object 9 in Figure~\ref{fig:cases}). In this case we want to maintain the one object ID and assign it to each of the regions.
      % \maneesh{How is occlusion different from collision. I think we want to be careful about these two terms.}
    \item \textbf{Many-to-many.} In some cases objects may break apart and merge in a larger group, resulting in a many-to-many mapping (see objects 5 and 6 and regions E and F in Figure~\ref{fig:cases}). Moreover, it may be unclear how to propagate the object IDs. We discuss how to handle this case Section~\ref{}. \maneesh{Not sure the example in Fig 4 is correct. Both elements in frame t-1 and t must consist of two objects. So we need 4 objects all together and there needs to be a flip in which ones are connected as a single region.}
\end{enumerate}
% \maneesh{Why is many-to-many missing from the list of cases?}
% \maneesh{alt: Note however that the mappings between shapes and regions is not always one-to-one. (May need to introduce all the cases we handle here -- many-to-one and one-to-many and explain why we don't need many-to-many.} 

To compute the assignment mapping we build a complete directed
bipartite graph $B = (\mathcal{S}_{t - 1}, \mathcal{R}_t)$.
\maneesh{Should explain what directions mean in the graph.}
Edges in the graph indicate a possible correspondence between an object and a region. Our approach is to remove the edges in this complete graph that represent unlikely correspondences, until only valid mappings remain.
% \maneesh{I think we should explain the parenthetical statement up
%   front in this subsection and remove the parens.}
% These correspondences will determine which object identifiers are propagated to which regions. 
% \maneesh{The correspondences don't directly
%   determine this. We use the correspondences as hypotheses for the
%   final mappings and the goal is to pick the ``best'' hypothesis.}
This occurs in two passes: first, we coarsely match
objects to regions using appearance and optical flow features
(Section\,\ref{sec:coarse_match}); then, we use differentiable compositing to determine our final mappings (Section\,\ref{sec:fine_match}). The goal of the first pass is to reduce the number of local minima for the optimization in the second pass. The optimization then removes any remaining unlikely correspondences. \maneesh{We will need to define differentiable compositing earlier and explain here why it is a good choice for the fine scale matching.}

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{skeleton_figs/coarse_mapping.png}
    \caption{Coarse mappings. \sharon{Is this figure necessary, or is the relevant text in \ref{sec:coarse_match} clear enough?}}
    \label{fig:coarse_mapping}
\end{figure}

\subsubsection{First edge removal pass}
\label{sec:coarse_match}
% Ultimately, we want to determine the exact position and location of
% each shape from frame $F_{t - 1}$ in frame $F_t$. This will be done by
% applying the differentiable compositing framework~\cite{} on
% shape-region correspondences, as described in the follow
% Section~\ref{fine_match}. However, this process requires a good
% initialization of the parameters being optimized, \ie we must make a
% good initial guess at the affine transformation to apply to an element
% in order to converge accurately to its target appearance.
% \maneesh{This paragraph seems out of place as it seems like a
%   higher-level abstract of the approach. Also we are in the
%   shape/region mapping section, so we want to focus on the specific
%   problem here of computing correspondence hypotheses.}

We begin by assigning weights to the edges in $B$ that describe how ``good" a correspondence is between an object and a region. This weight is determined by a combination of contour, appearance and motion features. Contours are represented using elliptic Fourier descriptors~\cite{}, appearances are represented with color histograms and motion is extracted from forward optical flow ($\overrightarrow{\mathcal{F}}_{t - 1}$) and backward optical flow ($\overleftarrow{\mathcal{F}}_t$). Contour and color allow us to compare objects visually, and the forward and backward flow provide pixel-level motion correspondences. More formally, the weight between a shape $S_i \in \mathcal{S}_{t - 1}$ and a region $R_j \in \mathcal{R}_t$ is defined as
% To provide the subsequent optimization with a good initialization, we first reduce the search space by deleting edges of $B$ that represent improbable correspondences.
% \maneesh{We should explain the general idea (e.g. the features we will be considering) before presenting the equation. Not sure
% how a weight allows us to delete edges.}
\begin{equation}
    w(S_i, R_j) = s_c(S_i, R_j) \cdot s_{\text{LAB}}(S_i, R_j) \cdot \frac{\overrightarrow{f}(S_i, R_j) + \overleftarrow{f}(S_i, R_j)}{2}.
\end{equation}
This weight is the product of four score functions. The first score $s_c$ is the inverse absolute cosine similarity between elliptic Fourier contour descriptors to 10 orders, or
\begin{equation}
  d_c(S_i, R_j) = 1.0 - | \langle \text{efd}(S_i), \text{efd}(R_j) \rangle |.
\end{equation}
The second score $s_\text{LAB}$ is a color similarity defined as
\begin{equation}
  d_\text{LAB}(S_i, R_j) = 1.0 - d_\text{Hel}(hist_\text{LAB}(S_i), hist_\text{LAB}(R_j)),
\end{equation}
where $hist_\text{LAB}$ is the LAB colorspace histograms using 64 bins per channel and $d_\text{Hel}$ denotes the Hellinger distance between two distributions.

The final score is an average of two values: the \textit{forward intersection} and \textit{backward intersection} scores. The forward intersection score describes how well an object and a region intersect according to the optical flow from time $t - 1$ to time $t$, computed using RAFT~\cite{} pretrained on the Sintel~\cite{} dataset. This gives us a rough idea of which regions are present in the area into which an object moves. The backward intersection score is defined similarly, from time $t$ to time $t - 1$. They are defined as
\begin{equation}
    \overrightarrow{f}(A, B) = |\overrightarrow{\mathcal{F}}_{t - 1}(A) \cap B|
\end{equation}
and
\begin{equation}
    \overrightarrow{\mathcal{F}}(A, B) = |A \cap \overleftarrow{\mathcal{F}}_t(B)|,
\end{equation}
respectively. Here, $\overrightarrow{\mathcal{F}}_{t - 1}$ and
$\overleftarrow{\mathcal{F}_t}$ denote the optical flow from frame
$F_{t - 1}$ to frame $F_t$ and vice versa, respectively.
\maneesh{Do we just use intersection or intersection over union?}
%  \maneesh{I
%   think we want to first explain why flow in the forward direction
%   with the intersection score can be used as a hypothesis. Then
%   explain why backwards flow is also useful, then talk about
%   appearance score. Build these up explain why each score is useful
%   and then give the form of the score as an equation and finally
%   combine all the scores into a weight.}
  % \maneesh{I think we should clarify that RAFT is just the optical flow computation, not the score computation -- right?}

The resulting score between an object $S_i$ and a region $R_j$ is assigned to both directed edges $S_i \rightarrow R_j$ and $S_i \leftarrow R_j$. Once all the edges have been assigned weights, we remove all edges which have a weight of 0.

\subsubsection{Second edge removal pass}
\label{sec:fine_match}
The first edge removal pass should remove a majority of the edges in
$B$. This may result in a set of ``connected'' components, where
connectivity is defined by an edge in any direction between two
nodes. For each connected component, we perform another round of edge
culling using an optimization pass that incorporates differentiable
compositing~\cite{}. We optimize over all affine parameters as well as
$z$-indexes to allow for layering. This allows us to (1) match objects
and regions in similar orientations \sharon{need to word this first
  point better} as well as (2) quantify how well those match-ups are
with a visual loss. \maneesh{Can shorten this paragraph.}

\maneesh{Start by explaining what a connected component consists of -- a set of objects that map to a set of regions (should refer to a figure). Then explain the goal we are trying to achieve with differential compositing. I think we are trying to find for each object a transformation mapping it to each of the regions and for each region a transformation mapping (``mapping'' is overloaded here) it to each of the objects. We start by computing the transformations for each object by optimizing the set of objects (treating them as sources) in the connected components against the regions (treating them as targets). We then do the reverse..}
The optimization proceeds as follows. For each connected component $C$
in $B$, we compute a target image consisting of all the regions in $C$
and mask out the other regions. We also compute a set of source
images, one corresponding to each object in $F_{t - 1}$. We
\textit{jointly} optimize the affine transformation and $z$-indexes of
all the objects against the target image. This joint optimization is
important because it allows for us to account for object
occlusions. \sharon{is it clear what I am emphasizing in the previous
  sentence?} Our loss function is a visual loss between the composited
transformed objects and the target image, so the optimization should
converge to a minimum that orients objects over the areas in the
target image which are most visually similar. This optimization is
performed twice for each component, once in the forward direction
(optimizing object orientations against a target image of regions in
$F_t$) and in the backward direction (optimizing region orientations
against a target image of objects in $F_{t - 1}$). This is to ensure
that we identify cases 4 and 6 in Figure~\ref{fig:cases}, as well as
the orientations of shapes that are partially off-frame.
\maneesh{Need to explain somewhere that we are extended Reddy to compute a shear.}


\maneesh{We should first explain why we need to modify Reddy's loss and then focus on how our modification helps our approach. In the writeup below it is unclear what Reddy's original loss was and what our modifications are.}
Our loss is adapted from Reddy~\etal~\cite{}. Given a target image
$I^*$ and the composited optimized image $I'$, we define the loss
\sharon{look up notation in DiffComp paper and match below}
\begin{equation}
  \mathcal{L} = \mathcal{L}_\text{scales} + \gamma * \mathcal{L}_\text{params}.
\end{equation}
The first loss term $\mathcal{L}_\text{scales}$ is an $L_2$ loss computed at multiple scales, 
\begin{equation}
  \mathcal{L}_\text{scales}(I', I^*) = \sum_{s=1}^K ||I'_s - I^*_s||_2
\end{equation}
\maneesh{Not sure we've defined all the variables in the eqn above.}
where $I_s$ denotes an image $I$ resized by a factor of $1/2$.

The second loss is a regularization term on the optimization variables
to encourage smaller orientation changes of objects between frames,
\begin{equation}
  \mathcal{L}_\text{params}(\mathbf{x}_t, \mathbf{x}_{t - 1}) = ||\mathbf{x}_t - \mathbf{x}_{t - 1}||_1.
\end{equation}
\maneesh{L1 loss typically encourages sparsity -- one bigger change rather than lots of small changes. Also it is not clear what the $x$ here are -- I think they are the transformation parameters. So this regularization loss is trying to encourage sparsity in the transformation parameters. But we may be running into an issue where the parameters are on different scales, so the loss may be doing some funny things. Finally we should say how $\gamma$ is set.}

Once the optimization has converged, we proceed to determine which
edges in $C$ we should keep. Only edges between objects and regions
which overlap significantly in the optimization result should be kept,
as this is an indication that those objects and regions correspond
visually.  \maneesh{Would be
  good to say we are removing edges rather than keeping them.}

\maneesh{I'm a bit confused by the remainder of this section.}  Assume
we are in the forward optimization (the backwards optimization case is
analogous). We begin with no edges in $C$ and iteratively add edges
that represent likely object-region correspondences. From the
optimization, we have a set of transformed objects. For each
transformed object $S_i \in C$ we compute the region
\begin{equation}
  R_{j^*} = \text{argmax}_{R_j \in C} |R_j \cap S_i| / |S_i|,
\end{equation}
\ie the region by which $S_i$ is maximally covered. \maneesh{alt: the region which most overlaps S.}
We also compute the set of regions
\begin{equation}
  \mathcal{R} = \{ R_j | |R_j \cap S_i| / |R_j| > 0.9, R_j \in C \},
\end{equation}
\ie the regions which are covered by $S_i$ by more than a fraction of 0.9. We add the edges $S_i \rightarrow R_{j^*}$ and $\{ S_i \leftarrow R_j, R_j \in \mathcal{R} \}$. This process is repeated for all connected components of $B$.
\maneesh{I don't follow how we are getting leftarrow edges from the forward computation. What does arrow direction signify?}


\maneesh{I wonder if we can simplify a lot of the next section by focusing on the transformations that are computed for each edge in the graph. If multiple objects overlap a region and have similar transformations we should be in the many-to-one-merge case. If multiple objects overlap a region but have different transformations, we should be in the many-to-one-nomerge case -- etc.}

\subsubsection{Propagating object IDs}

\sharon{This part needs a clarity check. I think there is too much notation here, but not sure how to reduce it. Do you think I can use the terms ``objects'' and ``regions'' without the corresponding $S_i$ and $R_j$'s?} After the second edge removal process, we use the remaining edges to determine what mappings in Figure~\ref{fig:cases} possibly occur. To identify potential mappings, we iterate through each node in $B$ and collect all possible mapping cases 1 through 5 involving that corresponding object or region. Each node in $B$ may contribute either a forward mapping, backward mapping, or both. For an object $S_i$, the forward mapping is the object and all regions $R_j$ for which the edge $S_i \rightarrow R_j$ exists. The backward mapping is the object and all regions $R_j$ for which the edge $S_i \leftarrow R_j$ exists. Similarly, for a region $R_j$ the forward mapping is the region and all objects $S_i$ for which the edge $S_i \rightarrow R_j$ exists, and the backward mapping is the region and all objects for which the edge $S_i \leftarrow R_j$ exists. Forward mappings include the one-to-one, many-to-one (no merge) and one-to-many (no split) mappings. Backward mappings include the one-to-one, many-to-one (merge) and many-to-one(split) mappings. Note that this does not include the many-to-many case--since we do not define an assignment of IDs for this case, we simply consider all other mappings that appear within the many-to-many case.
\maneesh{I'm confused by the difference between the arrow directions and the forward/backward mappings. Do we need to thing about both things?}

\begin{figure}
  \centering
  \includegraphics{figs/mapping_selection-02.png}
  \caption{Mapping selection.}
  \label{fig:mappings}
\end{figure}

\sharon{I think the following section may also be confusing. It really is meant to explain the significance of these forward/backward descriptors and how they relate to the forward/backward optimization passes.}
Each mapping also has an associated score that quantifies how well the objects and regions matched visually in the optimization process from the second edge removal process. The score is computed with a masked RGB $L_2$ loss as follows. First, we identify whether the mapping consists of edges that were added in a forward or backward optimization pass. A mapping $\mathcal{S} \rightarrow \mathcal{R}$ is from a forward pass, whereas a mapping $\mathcal{S} \leftarrow \mathcal{R}$ is from a backward pass. \sharon{Is the previous sentence obvious? Do I need it?} The mask for a ``from node,'' or a node from which an edge points out, is the mask of that object or region in the target image. The mask for a ``to node,'' or a node to which edges point in, is the mask of that object or region in the optimized composite image. We compute the combined (or operation) of all these masks and then compute the masked $L_2$ RGB loss between the optimized composite image and the target from that optimization pass; this loss is the final mapping score.

The result from the procedure above is a set of possible mappings. However not all the mappings can exist together--a forward mapping and backward mapping out of the same node, for example, will result in conflicting ID assignments. Thus, our next step is to select a subset of mappings which do not conflict. We do so in a greedy manner. We repeatedly select the mapping with the lowest score and perform the corresponding ID assignments for the regions in that mapping. Then, we remove all conflicting mappings from our set. A conflicting mapping is one which includes any nodes that a selected mapping already includes. Once all conflicting mappings have been removed, we repeat the process again. We stop once there are no more mappings left in our set \textit{or} the score of our best possible mapping is higher than some threshold. The threshold reduces the chances that we select a mapping which resulted from an optimization pass that converged to a suboptimal local minimum. An example mapping selection is described in Figure~\ref{fig:mappings}. The full mapping selection process is described in Algorithm~\ref{alg:mappings}. \sharon{Do I need both the algorithm and the figure?}

\begin{algorithm}
  \caption{Selecting valid mappings}\label{alg:mappings}
  $\text{Given a set of candidate mappings } \mathcal{M}, \alpha$;
  
  $\mathcal{M}^* \gets {}$;
  
  \While{$|\mathcal{M}| > 0$}
  {
      $M^* \gets \text{argmin}_{M \in \mathcal{M}} \texttt{score}(M)$;
  
      \For{$M \in \mathcal{M}$}{
          \If{$|\texttt{shapes}(M) \cap \texttt{shapes}(M^*)| > 0$ \text{ or } \\
          $|\texttt{regions}(M) \cap \texttt{regions}(M^*)| > 0$}{
              $\mathcal{M}. \texttt{remove}(M)$;
          }
      }
  
      \If{$\texttt{score}(M^*) > \alpha$}{
          $\mathcal{M}^*. \texttt{add}(M^*)$;
      }
  
      \Return{$\mathcal{M}^*$};
  }
  \end{algorithm}

Once we have our set of selected mapping, we assign IDs to regions
according to the specified rules at the beginning of
section~\ref{sec:pipeline_ii}. \maneesh{The cases at the beginning of Section 3.3 should be thought of as things that might happen -- not as rules. We should explicitly say how we propagate IDs for each case.}

\subsubsection{Canonical appearances}
During this stage, we also keep track of a canonical appearance for each object. The final motion parameters in our program will be computed with respect to this canonical appearance. We begin with the initial appearance of an object when
it is first identified. Whenever the same object is identified in a subsequent frame, we update the appearance if the object is unnoccluded and has a higher resolution than the current appearance.

% LocalWords:  efd Hel colorspace Hellinger pretrained Sintel Reddy
% LocalWords:  Reddy's DiffComp params eqn iteratively argmax RGB shp
% LocalWords:  leftarrow argmin unnoccluded mathcal clr advect RANSAC
% LocalWords:  et al de z's cmp vis centroid cov src tgt suboptimal


==> pipeline_iii.tex <==
\subsection{Motion recovery}\label{sec:pipeline_iii}
After the object identification stage, we obtain a set of object masks indicating the pixels covered by each object at each frame. The final step is to determine the motion parameters of the objects as they progress through the video. Our parameters include scale, rotation, skew and the coordinates of the object's bounding box centroid. For each object in a frame, we have the
canonical object appearance and the target object appearance
(determined by the object masks). 
We use the differentiable compositing optimization framework to determine the  motion parameters and z-index of each object, and these parameters are written out to the final program.
\maneesh{We probably need to explain why another optimization is necessary here. It seems like it shouldn't really need to be optimized again. Perhaps to get a little bit better fit. But I contend that it should be possible to get the transformations from the sequence of transformations that was computed frame to frame.}

==> results_eval.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=\textwidth]{figs/evaluation.pdf}
        % \vspace{-1.5em}

        \caption{We evaluate our motion vectorization pipeline by
          comparing the $L_2$ RGB error between input video frames and
          the same frame rendered with our extracted program (reconstruction).
          %Our per-frame reconstruction errors are comparable with the
          %  reconstruction errors in Reddy \etal~\cite{} \sharon{Is this
          %  necessary to state?}.
          \sharon{Note: Will recreate with alpha matting. Lighten up the diff color. Add another results column.}
          \maneesh{Not sure what alpha matting means, perhaps showing the source elements? I think that would be useful.}
        }
    \label{fig:eval}
\end{figure*}

\subsection{Evaluation}
\label{sec:eval}


We evaluate our generated programs using per-frame $L_2$ RGB
differences (Figure~\ref{fig:eval}) and a comparison of video and
program file sizes. Over a set of 21 videos \sharon{.mov videos}
totaling 1,842 frames, the average $L_2$ reconstruction error of our
output programs is $0.0179$ \sharon{Do we need to provide context
  about where the videos came from?}. The average size of each of
these videos is 4.80MB and size of the corresponding programs is
11.51\% of the input video on average. \sharon{Is a table of the
  video/program file sizes for all of these videos necessary?}
\maneesh{I don't think we need a table. I would brighten the diff image a bit. I wonder if we need the scale on the diff image. }

% \sharon{Table of reconsruction errors}
% \sharon{Results figure showing original, reconstruction and diff}
% \sharon{Potential baselines (nice to have)}
%\maneesh{Maybe compare size of SVG program to size of input motion graphics video as compactness of our representation is a plus.}
% baselines


==> sharon_equations.tex <==
\sharon{
\subsection{Differentiable Compositing}
$M^\text{vis}(S_i, \mathcal{C}(\mathcal{S}^*))$ is the set of pixels of $\Theta_i(S_i)$ which are visible in $\mathcal{C}(\mathcal{S}^*)$. 

\subsection{Stage 2: Generate candidate mapping types}
For the forward optimization direction, we have $DC(\mathcal{O}_{t - 1}, F_t) = \mathcal{O}^*_{t - 1}$. We compute a \textit{source} coverage weight with respect to $\mathcal{O}^*_{t - 1}$ and $F_t$ as
\begin{equation}
   W^\text{src}_{cov}(O_i, R_j) = \frac{|M^\text{vis}(O_i, \mathcal{C}(\mathcal{O}^*_{t - 1})) \cap M^\text{vis}(R_j, F_t)|}{|M^\text{vis}(O_i, \mathcal{C}(\mathcal{O}^*_{t - 1}))|}
\end{equation}
and a \textit{target} coverage weight as
\begin{equation}
   W^\text{tgt}_{cov}(O_i, R_j) = \frac{|M^\text{vis}(O_i, \mathcal{C}(\mathcal{O}^*_{t - 1})) \cap M^\text{vis}(R_j, F_t)|}{|M^\text{vis}(R_j, F_t)|}.
\end{equation}
The coverage weights in the backwards directions are defined analogously with respect to $\mathcal{R}^*_t = DC(\mathcal{R}_t, F_{t - 1})$ and $F_{t - 1}$ as $W^\text{src}_{cov}(R_j, O_i)$ and $W^\text{src}_{tgt}(R_j, O_i)$.

\subsection{Stage 3: Score candidate mappings}
We define a loss score for a forward mapping  $(\tilde{\mathcal{O}}_{t - 1}, \tilde{\mathcal{R}}_t)$ with respect to $\mathcal{O}^*_{t - 1} = DC(\mathcal{O}_{t - 1}, F_t)$ and $F_t$ as 
\begin{equation}
    \mathcal{L}^\text{vis}(\tilde{\mathcal{O}}_{t - 1}, \tilde{\mathcal{R}}_t) = || M^\text{union} \otimes (\mathcal{C}(\mathcal{O}^*_{t - 1}) - F_t)||_2,
\end{equation}
where 
\begin{equation}
    M^\text{union} = M^\text{vis}(\tilde{\mathcal{O}}_{t - 1}, \mathcal{C}(\mathcal{O}^*_{t - 1})) \cup M^\text{vis}(\tilde{\mathcal{R}}_t, F_t).
\end{equation}
The definitions of $M^\text{vis}$ over the sets $\tilde{\mathcal{O}}_{t - 1}$ and $\mathcal{R}_t$ are the unions
\begin{equation}
    M^\text{vis}(\tilde{\mathcal{O}}_{t - 1}, \mathcal{C}(\mathcal{O}^*_{t - 1})) = \bigcup_{O_i \in \tilde{\mathcal{O}}_{t - 1}} M^\text{vis}(O_i, \mathcal{C}(\mathcal{O}^*_{t - 1}))
\end{equation}
and
\begin{equation}
    M^\text{vis}(\tilde{\mathcal{R}}_t, F_t) = \bigcup_{R_j \in \tilde{\mathcal{R}}_t} M^\text{vis}(R_j, F_t).
\end{equation}
The loss score for a backward mapping $(\tilde{\mathcal{R}}_t, \tilde{\mathcal{O}}_{t - 1})$ is defined analogously with respect to $\mathcal{R}^*_t$ and $F_{t - 1} = DC(\mathcal{R}_t, F_{t - 1})$.
}


==> system.tex <==
\section{System overview}
% Discuss motion graphics and what characterizes them.
% Is this necessary?
\label{sec:system}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{skeleton_figs/system.png}
    \caption{System overview}
    \label{fig:system}
\end{figure*}

Our program induction pipeline has three main parts, as shown in
Figure~\ref{fig:system}. The first module performs \textit{region
  extraction} on every frame of the input video. The per-frame region
information is then passed to an \textit{object identification} module which assigns
a unique identifier to regions corresponding to the same object and also extracts a canonical appearance for each object. This
resulting set of object mask layers and object appearances is passed
to the final \textit{motion recovery} module, which determines the affine
transformation applied to the object appearance at every frame.
% \maneesh{I think ``tracking'' is a term for the whole pipeline -- or
%   at least the part that computes frame to frame motions seems to be
%   the ``tracking'' component. I might change the names to (1) Region
%   Extraction, (2) Shape/Region Matching (or Shape/Region
%   Identification) and (3) Motion Tracking (or Motion/Warp
%   Recovery). Also we should look at related work to see if the
%   Tracking literature already names thees components.}

% The resulting program can be rendered to a browser with SVG or loaded
% into other editing software such as After Effects and Blender. In
% Section~\ref{sec:apps}, we also demonstrate some automated video
% editing tasks by applying certain functions to the \program itself and
% output a modified \program. \maneesh{At this point readers should know
% that we will show applications of the resulting SVGs later. I think we can remove it from here.}

Since the space of motion graphics videos covers a large variety of
visual effects, motions and transitions, we introduce a set of
assumptions on the objects and motions in our input videos.
\maneesh{I think the reasoning needs to be a bit more explicit in this paragraph. Motion graphics vary a lot, but a large class of them fit a few assumptions... Would be even stronger if we could explain why they fit these assumptions. My sense is that there is a large class of motion graphics videos that are 2D affine motions of solid colors, gradients and patterns formed from a small palette of colors. Can we find books on motion graphics that say this or something similar. Can we base this on examples?}

\begin{enumerate}
    \item \textbf{Clear visual boundaries.} New objects frequently
      appear and disappear at various points in motion graphics
      videos. In order to avoid burdening a user with the task of
      scrubbing through an entire video and indicating each unique
      object that appears, we opt to automatically extract unique
      objects. To reliably do so, we assume that all objects are
      bounded by a clear visual border and have no internal borders.
      \maneesh{I wouldn't worry about explaining why it would be herd for a user to specify boundaries. I think each of these bullets should explain why videos tend to follow these assumpitons -- visible boundaries allow viewers to visually/perceptually separate foreground objects from one another and from the background.}
    
    \item \textbf{Affine motion model.} We assume an affine model on
      the object's appearance. This is consistent with the basic
      features of video timeline editors in programs such as Adobe
      After Effects~\cite{} and \todo.
      \maneesh{I think it would be stronger motivation to explain why an affine model still allows a wide variety of videos and why so many videos fit this assumption. Also it is not clear that After Effects limits to affine motions -- it might allow homographics -- I'm not sure if non-uniform shears enable homographies. }
    
    \item \textbf{Uniform background region.} Since the video
      background typically will not adhere to an affine motion model,
      we perform foreground-background segmentation and only extract
      regions from the foreground. \todo.
      \maneesh{Why won't background adhere to affine motion? I think often it will. I think we should think about this limitation and whether we can remove it or at least partially remove it. What we need is a good background segmenter or matte extractor. Seems like there should be a few things to try here.}
      
\end{enumerate}

